A Fuzzy-Based Optimization Method for Integrating Value Dependencies into Software Requirement Selection

Software requirement selection aims to find an optimal subset of the requirements with the highest value while respecting the budget. But the value of a requirement may depend on the presence or absence of other requirements in the optimal subset. Existing requirement selection methods, however, do not consider Value Dependencies, thus increasing the risk of value loss. To address this, we have proposed Dependency-Aware Requirement Selection (DARS) method with two main components: (i) a fuzzy-based technique for identifying and modeling value dependencies, and (ii) an Integer Programming model that takes into account value dependencies in software requirement selection. We have further, proposed an alternative optimization model for situations where quantifying value dependencies is hard. The scalability of DARS and its effectiveness in reducing the risk of value loss are demonstrated through exhaustive simulations.

==> case.tex <==
\section{Case Study}
\label{ch_dars_validation_case}

This section discusses the practicality and validity of DARS by studying a real-world software project. We demonstrate why software vendors should take care with value dependencies among requirements, and how to employ DARS to assist decision makers to comprehend the results, thus raising the following research questions.

\input{rq/rq_dars_ilp_case}

==> case_description.tex <==
\subsection{Description of Study}
\label{ch_dars_validation_case_description}

To demonstrate the practicality of DARS, we studied a real-world software project. Table~\ref{table_ch_dars_cost_value} lists the requirements of the project and their estimated and expected values in $[1,20]$. The expected value of each requirement $r_i$, denoted by $E(v_i)$ was computed by multiplying the frequency of the presence of $r_i$ in the configurations of the project sold in the earlier versions of software ($p(r_i)$) by its estimated value $v_i$. 

\begin{table*}[!htbp]
	\caption{The estimated and expected values of the requirements.}
	\label{table_ch_dars_cost_value}
	\centering
	\input{ch_dars/tables/table_value}
\end{table*} 

Our study began with the identification of value dependencies and modeling those dependencies as depicted in Figure~\ref{fig_ch_dars_cs_design}. Then we performed requirement selection using PCBK, SBK, and DARS based on the sales records of the previously rleased configurations of software. For the configurations found by PCBK, SBK, and DARS (Figure~\ref{fig_ch_dars_selectionMap_pcbk_dars} and Figure~\ref{fig_ch_dars_cs_selectionMap_sbk_dars}), the accumulated value (AV), expected value (EV), and overall value (OV) were computed to compare the performance of those methods for different price levels. This helped stakeholders to find, for different price levels, configurations with lower risk of value loss.  

\begin{figure*}[!htbp]
	\centering\includegraphics[scale=0.235]{ch_dars/figs/fig_cs_design_new_3}
	\captionsetup{margin=2ex}
	\caption{%
		The case study design.
	}%
	\label{fig_ch_dars_cs_design}
\end{figure*}

%We moreover, avoided comparing configurations with different prices to prevent from the impact of price on the sales/revenue in our comparisons. Configurations recommended by PCBK method were not used at this stage as they only account for precedence dependencies (structural and semantic dependencies) among requirements while entirely ignoring user preferences. 
%------------------------------------------------------------------------------------------------------------------------------ 

==> case_identification.tex <==
\subsection{Identifying and Modeling Value Dependencies}
\label{ch_dars_case_identification}

To account for the precedence dependencies among the requirements of the project, dependencies of type \textit{Requires} and \textit{Conflicts-With} were extracted (Figure~\ref{fig_ch_dars_cs_precede}) from the development artifacts of the project and formulated as (\ref{eq_ch_dars_pcbk_cs_precedence_2})-(\ref{eq_ch_dars_pcbk_cs_precedence_14}) in the optimization models of PCBK, SBK, and DARS. Moreover, (\ref{eq_ch_dars_pcbk_cs_precedence_1}) was added to account fo the constraint that the presence of either $r_2$ or $r_6$ is always essential. $x_i$ denotes whether $r_i$ is selected ($x_i=1$) or not ($x_i=0$). 

\begin{figure*}[!htbp]
	\centering\includegraphics[scale=0.8]{ch_dars/figs/fig_cs_vertical}
	\vspace{-0.25cm}
	\caption{%
		The precedence dependency graph of the requirements.
	}%
	\label{fig_ch_dars_cs_precede}
\end{figure*}

\begin{align}
\label{eq_ch_dars_pcbk_cs_precedence_1}
&x_2 + x_6 =1\\
\label{eq_ch_dars_pcbk_cs_precedence_2}
&x_4\leq x_1 + x_2\\
\label{eq_ch_dars_pcbk_cs_precedence_3}
&x_5\leq x_1 + x_2\\
\label{eq_ch_dars_pcbk_cs_precedence_4}
&x_8\leq x_1 + x_2\\
\label{eq_ch_dars_pcbk_cs_precedence_5}
&x_8\leq x_{25}\\
\label{eq_ch_dars_pcbk_cs_precedence_6}
&x_{17}\leq (1-x_{18})\\
\label{eq_ch_dars_pcbk_cs_precedence_7}
&x_{18}\leq (1-x_{17})\\
\label{eq_ch_dars_pcbk_cs_precedence_8}
&x_{19}\leq x_2\\
\label{eq_ch_dars_pcbk_cs_precedence_9}
&x_{19}\leq x_6\\
\label{eq_ch_dars_pcbk_cs_precedence_10}
&x_{20}\leq x_2\\
\label{eq_ch_dars_pcbk_cs_precedence_11}
&x_{20}\leq x_6\\
\label{eq_ch_dars_pcbk_cs_precedence_12}
&x_{26}\leq x_{27}\\
\label{eq_ch_dars_pcbk_cs_precedence_13}
&x_{27}\leq x_{1}\\
\label{eq_ch_dars_pcbk_cs_precedence_14}
&x_{27}\leq x_{6}
\end{align}

To find value dependencies among the requirements of the project, we first collected sales records of different configurations of the project as explained earlier. Then the Eells measure of causal strength was computed for all pairs of requirements using Algorithm~\ref{ch_dars_alg_identification} to identify the strengths and qualities of causal relations among the requirements as explained in Section~\ref{ch_dars_identification_relations}. The significances of the identified relations were subsequently tested using the Odds Ratio at confidence level $95\%$ as explained in Section~\ref{ch_dars_identification_testing}. The strengths and qualities of explicit value dependencies were finally computed using the significant causal relations found and the fuzzy membership function of Figure~\ref{fig_ch_dars_membership_1} as given by~(\ref{Eq_ch_dars_strengthMeasure})-(\ref{Eq_ch_dars_qualityMeasure}). Algorithm~\ref{alg_ch_dars_strength} was used to infer implicit value dependencies and compute the overall strengths of positive and negative value dependencies in the value dependency graph (VDG) of the requirements. The influences of the requirements on the values of each other were then computed by (\ref{Eq_ch_dars_influence}). 

\begin{figure*}[!htbp]
	\centering
	\hspace{0.0cm}\includegraphics[scale=0.33]{ch_dars/figs/result/fig_dependencies}
	\captionsetup{}
	\caption{%
		Explicit value dependencies among the requirements. Row $i$ and column $j$ denotes quality and strength of a value dependency from requirement $r_i$ to $r_j$.
	}%
	\label{fig_ch_dars_dependencies}
\end{figure*}


\begin{figure*}[!htbp]
	\centering
	\hspace{0.0cm}\includegraphics[scale=0.33]{ch_dars/figs/result/fig_influences}
	\captionsetup{}
	\caption{%
		 Influences among the requirements: cell $i,j$ gives the influence of $r_j$ on $r_i$.
	}%
	\label{fig_ch_dars_influences}
\end{figure*}

Figure~\ref{fig_ch_dars_dependencies} shows the qualities and strengths of explicit value dependencies. The color of a cell at row $i$ and column $j$ specifies the quality and the strength of a value dependency from $r_i$ to $r_j$. Colors associated with positive (negative) numbers denote positive (negative) dependencies. Also, zero denotes the absence of any value dependency. Similarly, the positive or negative influences of the requirements on the values of each other are depicted in Figure~\ref{fig_ch_dars_influences}.

%The color map of Figure~\ref{fig_ch_dars_influences} was presented to stakeholders for their review, where no substantial disagreement were found. Influences with magnitude $<0.2$ however, were found difficult to attribute to the preferences of users by the stakeholders. They, however, decided to still consider those influences. 

==> case_release.tex <==
\subsection{Analysis of Sales and Revenue}
 
Requirement selection aims to optimize the value of software products. When comparing two requirement selection methods hence the one that finds requirement subsets with higher value prevails. To compare the effectiveness of requirement selection methods hence, we need to study the impact of using those methods on the actual value (manifested in terms of revenue, profit, or return). Such study however requires software vendors to invest on developing/maintaining different configurations of a software product based on different selection methods even if such investment is not economically worthwhile. This clearly is difficult to achieve in real-world software projects due to the complexities of developing/maintaining software. In other words, software vendors hesitate to invest on different configurations of a software product proposed by different selection methods when the effectiveness of those methods in real-world software projects is under investigation. 

We addressed this problem using a post-release analysis~\cite{karlsson2003post} approach which relies on the sales records of a highly configurable office software product referred to as PMS-III whose several different configurations have sold over years. The sales records of PMS-III were used to study the revenue provided by the configurations found by the SBK and DARS-ILP methods during the target sales period. This way we managed to measure the effectiveness of the experimented selection methods without imposing additional costs to the software development/maintenance. 

In doing so, we first performed requirement selection as discussed in Section~\ref{ch_dars_validation_case_selection} using the PCBK, SBK, and DARS-ILP methods to find optimal configurations of PMS-III based on the sales records of different configurations of PMS-III sold prior to the target sales period (Pre-TSP). We then searched in the sales records of PMS-III for price levels at which the configurations found by the DARS-ILP and SBK methods (Figure~\ref{fig_ch_dars_cs_selectionMap_sbk_dars}) were amongst the frequently sold configurations during the four quarters of the target sales period (TSP). 

Those price levels include $\%Price=\{24,51,72,100\}$. We labeled configurations found by the SBK and DARS-ILP methods with $Price=24\%$ as \textit{Bronze} edition of PMS-III, configurations with $Price=51\%$ as \textit{Silver} edition, configurations with $Price=72\%$ as \textit{Gold} edition, and finally configurations with $Price=100\%$ were labeled as \textit{Ultimate} edition. For each edition and its corresponding configurations the details of sales and revenue was extracted from the TSP sales records and used to investigate the impact of using the SBK and DARS-ILP methods on the sales and revenue. 

Configurations found by the PCBK method were not used at this stage as they only account for precedence dependencies (structural and semantic dependencies) among requirements while entirely ignoring user preferences and value dependencies among requirements. Also, the Ultimate edition of PMS-III ($\%Price=100$) comprised the same subset of requirements in both SBK and DARS-ILP (Figure~\ref{fig_ch_dars_selection_100}) thus excluded from our analysis.

\begin{figure*}[!htbp]
	\centering
	\hspace{0.0cm}\includegraphics[scale=1,angle=90]{ch_dars/figs/result/fig_cs_selectionMap_sbk_dars}
	\captionsetup{margin=4cm}
	\vspace{-0.1cm}
	\captionsetup{margin=8ex}
	\vspace{0.5cm}
	\caption{%
		Requirement subsets found by the DARS-ILP method for different price levels compared to the ones found by the SBK method. 
	}%
	\label{fig_ch_dars_cs_selectionMap_sbk_dars}
\end{figure*}

%\begin{figure*}[!htbp]
%	\centering
%	\hspace{0.0cm}\includegraphics[scale=1.1,angle=90]{ch_dars/figs/result/fig_selectionMap_pcbk_dars}
%	\captionsetup{margin=4cm}
%	\vspace{-0.1cm}
%	\captionsetup{margin=8ex}
%	\vspace{0.5cm}
%	\caption{%
%		Requirement subsets found by the DARS-ILP method for different price levels compared to the ones found by the PCBK method. 
%	}%
%	\label{fig_ch_dars_selectionMap_pcbk_dars}
%\end{figure*}

% Four different editions of software labeled as \textit{Bronze}, \textit{Silver}, \textit{Gold}, and \textit{Ultimate} each released at a specific price level; $\%$Price(Bronze)=$25$, $\%$Price(Silver)=$50$, $\%$Price(Gold)=$75$, $\%$Price(Ultimate)=$100$. For each edition of PMS-III, two different editions of software \textcolor{red}{released, based on SBK and DARS-ILP methods} (Figure~\ref{fig_ch_dars_selection}). %Increase-Decrease models (Table~\ref{table_lr}) were not used due to their practical limitations as discussed in details in Section~\ref{sec_related}. Stakeholder also did not use PCBK model as it entirely ignores user preferences. 

\vspace{0.1cm}
\begin{figure*}[htbp]
	\begin{center}
		\subfigure[Bronze edition; $\%$Price=24]{%
			\label{fig_ch_dars_selection_25}
			\includegraphics[scale=0.65]{ch_dars/figs/result/fig_selection_24}
		}
		\subfigure[Silver edition; $\%$Price=51]{%
			\label{fig_ch_dars_selection_50}
			\includegraphics[scale=0.65]{ch_dars/figs/result/fig_selection_51}
		}
		\subfigure[Gold edition; $\%$Price=72]{%
			\label{fig_ch_dars_selection_75}
			\includegraphics[scale=0.65]{ch_dars/figs/result/fig_selection_72}
		}
		\subfigure[Ultimate edition; $\%$Price=100]{%
			\label{fig_ch_dars_selection_100}
			\includegraphics[scale=0.65]{ch_dars/figs/result/fig_selection_100}
		}
	\end{center}
	\captionsetup{margin=5ex}
	\caption{%
		Editions of PMS-III released by the PCBK, SBK, and DARS-ILP methods. Requirements are specified by their indexes. %For a given method, a gray-colored cell denotes presence of the corresponding requirement in the edition of software configured by that method. 
	}%
	\label{fig_ch_dars_selection}
\end{figure*}

The quarterly sales percentages of different editions of PMS-III and their corresponding configurations found by DARS-ILP and SBK are depicted in Figure~\ref{fig_ch_dars_sales_quarters_pie}. These percentages are computed by dividing the quarterly sales volume of each edition (configuration) by the total sales volume of all editions (configurations) found by DARTS-ILP and SBK in that sales quarter and multiplying the result by $100$. 
    
\begin{figure*}[htbp]
	\centering\includegraphics[scale=1.2]{ch_dars/figs/result/fig_sales_quarters_pie}
	\captionsetup{margin=8ex}
	\caption{Quarterly $\%$Sales for editions of PMS-III.}
	\label{fig_ch_dars_sales_quarters_pie}
\end{figure*}

\subsubsection{Analysis of Sales}

We observed that, in all sales quarters, the sales percentage of the Silver edition was higher than those of the Bronze and Gold editions. Configurations of the Silver edition found by the DARS-ILP method (Silver-DARS) sold around $9\%$, $15\%$, $12.2\%$, and $20.4\%$ higher than the configurations of the Silver edition found by the SBK method (Silver-SBK) in the \textcolor{red}{$1^{st}$ to $4^{th}$ sales quarters respectively}. In total, Silver-DARS \textcolor{red}{sold $14.87\%$ more} than Silver-SBK as in Figure~\ref{fig_ch_dars_sales_revenue_all}.

For the Bronze edition, Bronze-DARS sold around $2.5\%$, $6\%$, and $3.6\%$ more than Bronze-SBK during the quarters 2 to 4 respectively. In the first quarter however, sales percentages of Bronze-SBK and Bronze-DARS were almost equal. In total, the Bronze-DARS sold $3.3\%$ more than Bronze-PCBK as shown in Figure~\ref{fig_ch_dars_sales_revenue_all}. 

Similarly, for the Gold edition the sales percentages of Gold-DARS was $5.13\%$, $3.26\%$, $9.15\%$, and $13.83\%$ higher than that of Gold-SBK in the $1^{st}$ to $4^{th}$ sales quarters respectively. In total, Gold-DARS sold around $8.3\%$ more than Gold-SBK. 

In general configurations of PMS-III found by the DARS-ILP method sold more than the configurations found by the SBK method based on the sales record of the target sales period (TSP). This was more notable for the configurations found for Silver and Gold editions of PMS-III. Our results thus suggested that using the DARS-ILP method results in higher sales (this answers \textbf{RQ7}). 

\begin{figure*}
	\centering\includegraphics[scale=1.2]{ch_dars/figs/result/fig_revenue_quarters_pie}
	%\captionsetup{justification=centerlast, margin=10ex, labelfont=bf, textfont=it, format=plain, labelformat=default, labelsep=endash, font=small, name=Gráfico\,}
	\captionsetup{margin=10ex}
	\caption{Quarterly $\%$Revenue for editions of PMS-III.}
	\label{fig_ch_dars_revenue_quarters}
\end{figure*}


\subsubsection{Analysis of Revenue}

%Constraints (\ref{Eq_ch_dars_sbk_cs_c1}) and (\ref{Eq_ch_dars_dars_cs_c1}) in the optimization models of the SBK and DARS-ILP methods ensure that each configuration of PMS-III is found at a specific price level. This implies that a configuration with highr sales volume also provides higher revenue. Hence, Figure~\ref{fig_ch_dars_sales_quarters_pie} is sufficient by itself to demonstrate the advantage of using DARS-ILP in providing higher sales and consequently higher revenue. 

We observed (Figure~\ref{fig_ch_dars_sales_quarters_pie} and Figure~\ref{fig_ch_dars_sales_revenue_all}) that for all sales quarters the configurations of PMS-III found by the DARS-ILP method (Bronze-DARS, Silver-DARS, and Gold-DARS), provided (almost) equal or higher revenue compared to their corresponding configurations found by the SBK method (Bronze-SBK, Silver-SBK, and Gold-SBK). In total, Silver-DARS provided almost $15\%$ higher revenue compared to Silver-SBK and Gold-DARS provided almost $9.4\%$ higher revenue compared to Gold-SBK. Bronze edition of PMS-III released based on the DARS-ILP method (Bronze-DARS) also provided around $2\%$ higher revenue compared to Bronze-SBK. 

The total revenue achieved from different selection methods for different editions of PMS-III was consistent with the results of our selection tasks in Section~\ref{ch_dars_validation_case_selection}, where DARS-ILP provided higher overall value, at all price levels, compared to the SBK method (Figure~\ref{fig_ch_dars_ov_delta_dars_sbk}) by considering value dependencies identified from user preferences. SBK on the contrary, ignored value dependencies resulting in higher risk of value loss over the target sales period (TSP). This was observed for all editions of PMS-III.

\textbf{RQ8} hence can be answered by Figure~\ref{fig_ch_dars_sales_revenue_all} which demonstrates the advantage of using DARS-ILP in considering value dependencies by providing higher revenue for the Bronze, Silver, and Gold editions respectively over four sales quarters. Therefore, considering value dependences by the DARS-ILP method and using overall value as the measure of optimality in DARS-ILP resulted in configurations found by the DARS-ILP method to provide higher revenue compared to the configurations found by the SBK method. 

\begin{figure*}
	\centering\includegraphics[scale=1.2]{ch_dars/figs/result/fig_sales_revenue_all_pie}
	%	\captionsetup{justification=centerlast, margin=10ex, labelfont=bf, textfont=it, format=plain, labelformat=default, labelsep=endash, font=small, name=Gráfico\,}
	\captionsetup{margin=8ex}
	\caption{Percentages of sales/revenue achieved from different editions of PMS-III released by DARS-ILP and SBK in a one-year period.}
	\label{fig_ch_dars_sales_revenue_all}
\end{figure*}

==> case_selection.tex <==
\subsection{Performing Requirement Selection}
\label{ch_dars_validation_case_selection}

This section demonstrates the effectiveness of DARS in considering value dependencies compared to BK, PCBK and SBK methods. As discussed in Section~\ref{sec_related_pcbk}, PCBK considers the estimated values of requirements while SBK, as in Section~\ref{sec_related_sbk}, accounts for user preferences for requirements by considering the expected values of requirements rather than their estimated values. Finally, DARS method factors in both user preferences and value dependencies among requirements as explained in Section~\ref{ch_dars_selection_ilp}. The expected values of the requirements and value dependencies among them are computed based on the user preferences achieved from the sales records of the project.  

\begin{align}
\label{eq_ch_dars_pcbk_cs_c1}
&\sum_{i=1}^{27} v_i  x_i \leq \gamma 
\end{align}

Price was determined as a major constraint for requirement selection as different configurations of the project had been released at different price levels earlier to cope with the needs of different users~\cite{karpoff1987relation}. Constraints (\ref{eq_ch_dars_pcbk_cs_c1}) hence was added to the optimization models of PCBK, SBK, and DARS respectively to contain the price of different configurations of software within their corresponding price limits. This converted the problem to a variation of Bounded Knapsack Problem. $\gamma$ $\in {\rm I\!R^+}$ denotes the price limit and $v_i$ specifies the estimated value of a requirement $r_i$. Also $x_i$ specifies whether a requirement $r_i$ is selected ($x_i=1$) or not ($x_i=0$). We omitted (\ref{eq_sbk_c1}) from the optimization model of SBK as considering the sales diversification is beyond the scope of this paper. The concept of diversification was explained in detail in Section~\ref{sec_related}. 

\begin{figure*}[!htbp]
	\centering
	\hspace{-1.1cm}\includegraphics[scale=0.52,angle=0]{ch_dars/figs/result/fig_selectionMap_pcbk_dars}
	\caption{%
		 Requirement subsets found by DARS and PCBK for different price levels. 
	}%
	\label{fig_ch_dars_selectionMap_pcbk_dars}
\end{figure*}

\begin{figure*}[!htbp]
	\centering
	\hspace{-1.1cm}\includegraphics[scale=0.52,angle=0]{ch_dars/figs/result/fig_selectionMap_sbk_dars}
	\caption{%
		 Requirement subsets found by DARS and SBK for different price levels. 
	}%
	\label{fig_ch_dars_cs_selectionMap_sbk_dars}
\end{figure*}



Selection tasks were performed for different price levels ($\%\text{Price}=\{1,...,100\}$, $\text{Price} = \frac{\%\text{Price} }{100}\times 342$) using the optimization models of PCBK, SBK, and DARS with (\ref{eq_ch_dars_pcbk_cs_precedence_1})-(\ref{eq_ch_dars_pcbk_cs_precedence_14}) to find optimal subsets of the requirements (optimal configurations). Optimal configurations found by PCBK, SBK, and DARS were compared based on their similarities, accumulated values, expected values, and overall values to answer \protect\hyperlink{RQ1}{(\textbf{RQ1})} and its subquestions. Binary knapsack (BK) method (Section~\ref{sec_related_bk}) and the Increase-Decrease method (Section~\ref{sec_related_pcbk_CS}) were not used in the requirement selection tasks as the former ignores precedence dependencies resulting in violation of the precedence constraints while the latter does not provide any formal way to specify the amounts of the increased or decreased values of the requirement subsets as detailed in Section~\ref{sec_related_pcbk_CS}. Selections were performed using the callable library ILOG CPLEX 12.6.2 on a windows machine with a Core i7-2600 3.4 GHz processor and 16 GB of RAM.

%\improvement[inline]{More graphs?}

\subsubsection{Similarities of the Solutions} 
\label{ch_dars_validation_case_selection_comparing}

In this section, we compare PCBK, SBK, and DARS based on their selection patterns to answer \protect\hyperlink{RQ1.1}{(\textbf{RQ1.1})}. Figure~\ref{fig_distance} depicts dissimilarities between the requirement subsets found by the DARS and those found by PCBK/SBK based on \textit{Euclidean Distance}. While notable at all price levels, these dissimilarities decreased for highly expensive ($\%\text{Price} \rightarrow 100$) or very cheap ($\%\text{Price} \rightarrow 0$) configurations of the project. The reason is expensive configurations of software comprise most requirements thus reducing the chances that requirements with positive influences on the values of the selected requirements are ignored.

\begin{figure*}[htbp]
	\begin{center}
		\subfigure[DARS vs. PCBK]{%
			\label{fig_distance_minkowski}
			\includegraphics[scale=0.46]{ch_dars/figs/result/fig_cs_distance_dars_pcbk}
		}
		\subfigure[DARS vs. SBK]{%
			\label{fig_distance_euclidean}
			\includegraphics[scale=0.46]{ch_dars/figs/result/fig_cs_distance_dars_sbk}
		}
	\end{center}
	\captionsetup{margin=0ex}
	\vspace{-0.3cm}
	\caption{%
		Dissimilarities of the solutions found by DARS and PCBK/SBK. 
	}%
	\label{fig_distance}
\end{figure*}

Moreover, there are no negative influences among requirements (Figure~\ref{fig_ch_dars_influences}). Hence, similarities between solutions found by the DARS method and those found by PCBK and SBK increase for expensive configurations of software. For cheaper configurations, price constraint limits the solution space for PCBK, SBK, and DARS especially preventing the DARS method from utilizing its advantage in considering value dependencies. This resulted in more similarities between the solutions found by the DARS method and those found by PCBK and SBK for very cheap configurations of software. 

Finally, we observed from Figure~\ref{fig_ch_dars_selection_dars_pcbk} and Figure~\ref{fig_ch_dars_selection_dars_sbk} that the requirement subsets (solutions) found by DARS were more similar to the solutions found by SBK than similar to the solutions found by PCBK. The reason is as explained before both DARS and SBK consider user preferences while PCBK ignores those preferences. 

%\begin{figure*}[]
%	\centering\hspace{-0.3cm}\includegraphics[scale=0.48]{ch_dars/figs/result/fig_ch_dars_selectionMap}
%	\caption{%
%		Requirement subsets found by the PCBK and DARS-ILP models at different price levels. Color of a cell at row $i$ and column $j$ denotes whether the requirement $r_i$ is selected or ignored by either or both the PCBK and DARS-ILP models for $\%\text{Price}=j$.
%	}%
%	\label{fig_ch_dars_selection_map}
%\end{figure*}


\begin{figure*}[htbp]
	\begin{center}
		\subfigure[DARS vs. PCBK]{%
			\label{fig_ch_dars_selection_dars_pcbk}
            \hspace{-0.35cm}\includegraphics[scale=0.57]{ch_dars/figs/result/fig_selection_dars_pcbk}
		}
		\subfigure[DARS vs. SBK]{%
			\label{fig_ch_dars_selection_dars_sbk}
            \hspace{-0.35cm}\includegraphics[scale=0.57]{ch_dars/figs/result/fig_selection_dars_sbk}
		}
	\subfigure[SBK vs. PCBK]{%
		\label{fig_ch_dars_selection_sbk_pcbk}
		\hspace{-0.35cm}\includegraphics[scale=0.57]{ch_dars/figs/result/fig_selection_sbk_pcbk}
	}
	\end{center}
	\captionsetup{margin=0ex}
	\caption{%
		Selection patterns of PCBK, SBK, and DARS at different price levels. For a requirement $r_i$, denoted by $i$ on the x-axis, and requirement selection methods $m_j$ and $m_k$, $\%\Delta \text{F}_{i}(m_j,m_k) = \%\text{F}_i (m_j)-\%\text{F}_i (m_k)$, where $\%\text{F}_i (m_j)$ and $\%\text{F}_i (m_k)$ give the percentage of the selection tasks in which $r_i$ is selected by $m_j$ and $m_k$ respectively. 
	}%
	\label{fig_ch_dars_selection}
\end{figure*}

Figure~\ref{fig_ch_dars_selection} provides more insights into \protect\hyperlink{RQ1.1}{(\textbf{RQ1.1})} by comparing the selection patterns of PCBK, SBK, and DARS in $100$ different selection tasks performed at different price levels ($\%\text{Price}=\{1,2,...,100\}$). For a given requirement $r_i$, $\%\text{F}_i (m_j)$ specifies the percentages of the selection tasks in which $r_i$ is selected by requirement selection method $m_j$. Hence, $\%\Delta \text{F}_{i}(m_j,m_k) = \%\text{F}_i (m_j)-\%\text{F}_i (m_k) >0 $ states that the percentages of the selection tasks where $r_i$ is selected by $m_j$ is higher than the percentages of the selection tasks where $r_i$ is selected by $m_k$. Similarly, $\%\Delta \text{F}_{i}(m_j,m_k) = \%\text{F}_i (m_j)-\%\text{F}_i (m_k) <0 $ states that $r_i$ is more frequently selected by $m_k$ compared to $m_j$. $m_j$ and $m_k$ can be any of the selection methods used in our selection tasks. 

We observed (Figure~\ref{fig_ch_dars_selection}) that requirements with significant influence on the values of pricey requirements were more frequently preferred by DARS compared to PCBK and SBK. This was more visible for requirements $r_8$, $r_{12}$, $r_{24}$, and $r_{27}$ when in Figure~\ref{fig_ch_dars_selection_dars_pcbk} and for requirements $r_8$, $r_{12}$, $r_{24}$ in Figure~\ref{fig_ch_dars_selection_dars_sbk}. 

Requirement $r_8$, for instance, was more frequently preferred by DARS compared to PCBK and SBK as the optimization model of DARS considers the fact that $r_8$ has a significant positive influence on the values of several valuable requirements including $r_2$, $r_4$, $r_6$, and $r_{12}$ (Figure~\ref{fig_ch_dars_influences}). Similarly, $r_{24}$ has a significant (positive) influence on the values of requirements $r_2$, $r_6$, $r_8$, and$r_{12}$. $r_{25}$ however, was more frequently selected by DARS as $r_8$ requires $r_{25}$ (Figure~\ref{fig_ch_dars_cs_precede}) and $r_8$ is frequently selected by DARS due to its significant impact on valuable requirements. As such, selecting $r_8$ requires the presence of $r_{25}$ in software. DARS and SBK however were frequently selected $r_{12}$ and $r_{27}$ as these two requirements are almost always preferred by users. This was not the case for PCBK as it ignores user preferences.   

Selection patterns in Figure~\ref{fig_ch_dars_selection} showed that when a decision was to be made regarding the presence or absence of a requirement $r_i$ in a configuration of software, PCBK only took into account the estimated value of $r_i$ ignoring user preferences. SBK on the other hand, considered user preferences for $r_i$ by evaluating the expected value of $r_i$ rather than merely its accumulated value. 

DARS, however, considered the expected value of $r_i$ and the impact of $r_i$ on the values of other requirements. More similarities were, therefore, observed among the configurations found by SBK and DARS as both methods took into account user preferences. On the contrary, dissimilarities were more visible when SBK and DARS/PCBK were compared as demonstrated in Figure~\ref{fig_ch_dars_selection_dars_pcbk} and Figure~\ref{fig_ch_dars_selection_sbk_pcbk}.   

\subsubsection{Impact of DARS on the Overall Value} 

\protect\hyperlink{RQ1.2}{(\textbf{RQ1.2})} is answered by comparing the percentages of overall values ($\%\text{OV}=(\text{OV}/342)\times 100$), accumulated values ($\%\text{AV}=(\text{AV}/342)\times 100$), and estimated values ($\%\text{EV}=(\text{EV}/342)\times 100$) provided by PCBK, SBK, and DARS for $100$ selection tasks, each performed at a specific price level ($\%\text{Price}=\{1,2,..,100\}$), as shown in Figures \ref{fig_ch_dars_ov}-\ref{fig_ch_dars_ev}. Our results show (Figure~\ref{fig_ch_dars_ov}) that requirement subsets found by DARS provided higher or equal $\%$OV in all selection tasks compared to the PCBK method. The reason is that the optimization model of PCBK ignores user preferences and value dependencies among the requirements.

\begin{figure*}[htbp]
	\begin{center}
		\subfigure[]{%
			\label{fig_ch_dars_ov_all}
			\includegraphics[scale=0.46]{ch_dars/figs/result/fig_cs_ov}
		}
		\subfigure[]{%
			\label{fig_ch_dars_ov_delta_dars_pcbk}
			\includegraphics[scale=0.46]{ch_dars/figs/result/fig_cs_ov_delta_dars_pcbk}
		}
		\subfigure[]{%
			\label{fig_ch_dars_ov_delta_dars_sbk}
			\includegraphics[scale=0.46]{ch_dars/figs/result/fig_cs_ov_delta_dars_sbk}
		}
		\subfigure[]{%
			\label{fig_ch_dars_ov_delta_sbk_pcbk}
			\includegraphics[scale=0.46]{ch_dars/figs/result/fig_cs_ov_delta_sbk_pcbk}
		}
	\end{center}
	\captionsetup{margin=0ex}
	\vspace{-0.5cm}
	\caption{%
		Comparing the overall values at different price levels. $\%\Delta \text{OV}(m_j,m_k) = \%\text{OV}(m_j)-\%\text{OV}(m_k)$, where $m_j$ denotes a selection method (DARS, PCBK, or SBK).  
	}%
	\label{fig_ch_dars_ov}
\end{figure*}

For a given price, $\%OV$ of the requirement subset (solutions) found by the SBK method was, for most price levels, higher than $\%OV$ of the solution provided by the PCBK method but still less than or equal to the overall value of the solution found by DARS. The reason is that even though the SBK method does not consider value dependencies, it still accounts for user preferences, similar to DARS, by optimizing the expected values of selected requirements. This results in more similarities between the configurations found by the SBK method and those found by DARS as discussed in Section~\ref{ch_dars_validation_case_selection_comparing}. 

We observed in Figure~\ref{fig_ch_dars_ov_delta_dars_pcbk} that the gap between the $\%$OV achieved from DARS and the PCBK/SBK method was notable in almost all selection tasks performed at different price levels. But the gap reduced to almost negligible for highly expensive ($\%\text{Price} \rightarrow 100$) or very cheap ($\%\text{Price} \rightarrow 0$) configurations. The reason is, on one hand, there are no negative influences among the requirements (Figure~\ref{fig_ch_dars_influences}) and, on the other hand, expensive configurations of software comprise most requirements, which reduces the chances that requirements with positive influence are ignored by PCBK/SBK. 

\begin{figure*}[!htbp]
	\begin{center}
		\subfigure[]{%
			\label{fig_ch_dars_av_all}
			\includegraphics[scale=0.459]{ch_dars/figs/result/fig_cs_av}
		}
		\subfigure[]{%
			\label{fig_ch_dars_av_delta_dars_pcbk}
			\includegraphics[scale=0.459]{ch_dars/figs/result/fig_cs_av_delta_dars_pcbk}
		}
		\subfigure[]{%
			\label{fig_ch_dars_av_delta_dars_sbk}
			\includegraphics[scale=0.456]{ch_dars/figs/result/fig_cs_av_delta_dars_sbk}
		}
		\subfigure[]{%
			\label{fig_ch_dars_av_delta_sbk_pcbk}
			\includegraphics[scale=0.456]{ch_dars/figs/result/fig_cs_av_delta_sbk_pcbk}
		}
	\end{center}
	\captionsetup{margin=0ex}
	\vspace{-0.5cm}
	\caption{%
		Comparing the accumulated values at different price levels. $\%\Delta \text{AV}(m_j,m_k) = \%\text{AV}(m_j)-\%\text{AV}(m_k)$, where $m_j$ denotes a selection method (DARS, PCBK, or SBK).  
	}%
	\label{fig_ch_dars_av}
\end{figure*}


That increases similarities between the expensive configurations found by PCBK/SBK and DARS as discussed in Section~\ref{ch_dars_validation_case_selection_comparing}. For cheaper configurations, the price-constraint limited the solution space in all the PCBK, SBK, and DARS and specially prevented DARS from utilizing its advantage in considering value dependencies. The price constraint further reduced the gap between $\%$AV provided by DARS and PCBK/SBK (Figures~\ref{fig_ch_dars_av}) in the selection tasks.

We further, observed insignificant differences amongst the accumulated values provided by the selection methods experimented in this study as shown in Figure~\ref{fig_ch_dars_av}. The reason is that the price constraint in the optimization models of the PCBK, SBK, and DARS contain the accumulated values of the solutions found by those models. The price constraint is needed to factor out the interplay between the price and sales as explained earlier. Moreover, the expected values of the requirement subsets found by the SBK method were higher than those found by DARS and PCBK in all selection tasks (for all price levels) as shown in Figure~\ref{fig_ch_dars_ev_delta_dars_sbk} and Figure~\ref{fig_ch_dars_ev_delta_sbk_pcbk} respectively. 

\begin{figure*}[htbp]
	\begin{center}
		\subfigure[]{%
			\label{fig_ch_dars_ev_all}
			\includegraphics[scale=0.46]{ch_dars/figs/result/fig_cs_ev}
		}
		\subfigure[]{%
			\label{fig_ch_dars_ev_delta_dars_pcbk}
			\includegraphics[scale=0.46]{ch_dars/figs/result/fig_cs_ev_delta_dars_pcbk}
		}
		\subfigure[]{%
			\label{fig_ch_dars_ev_delta_dars_sbk}
			\includegraphics[scale=0.46]{ch_dars/figs/result/fig_cs_ev_delta_dars_sbk}
		}
		\subfigure[]{%
			\label{fig_ch_dars_ev_delta_sbk_pcbk}
			\includegraphics[scale=0.46]{ch_dars/figs/result/fig_cs_ev_delta_sbk_pcbk}
		}
	\end{center}
	\captionsetup{margin=0ex}
	\caption{%
		Comparing the accumulated values at different price levels. $\%\Delta \text{EV}(m_j,m_k) = \%\text{EV}(m_j)-\%\text{EV}(m_k)$, where $m_j$ denotes a selection method (DARS, PCBK, or SBK).  
	}%
	\label{fig_ch_dars_ev}
\end{figure*}

The expected values of requirement subsets found by DARS were higher than those of the requirement subsets found by the PCBK method in most selection tasks (Figure~\ref{fig_ch_dars_ev_delta_dars_pcbk}). In some of the selection tasks, however, the expected values of the requirement subsets found by the PCBK method were higher than those found by DARS even though the PCBK method does not account for user preferences. The reason is that DARS optimizes the overall value of a requirement subset (solution), which accounts for both user preferences and value dependencies. Hence in some cases DARS may find solutions with lower expected values as taking into account value dependencies may be in conflict with maximizing the expected values of a requirement subset. 


\subsubsection{Understanding the Conflicting Objectives} 

To answer \protect\hyperlink{RQ1.3}{(\textbf{RQ1.3})}, we compared the overall values (Figure~\ref{fig_ch_dars_ov}), accumulated values (Figure~\ref{fig_ch_dars_av}), and expected values (Figure~\ref{fig_ch_dars_ev}) of the requirement subsets found by the PCBK, SBK, and DARS in different requirement selection tasks performed at different price levels. From Figure~\ref{fig_ch_dars_ov} and Figure~\ref{fig_ch_dars_av} it can be seen that maximizing the accumulated value (AV) of a selected subset of requirements conflicts with maximizing the overall value (OV) of that subset. This can be specially seen in Figure~\ref{fig_ch_dars_ov_delta_dars_pcbk} and Figure~\ref{fig_ch_dars_av_delta_dars_pcbk}, where in several selection tasks, choosing requirement subsets with higher $\%$AV by the PCBK method (Figure~\ref{fig_ch_dars_av}) reduced the overall value. 

Maximizing the expected value of a requirement subset also conflicts with optimizing its overall value as the former may result in ignoring requirements with lower expected values even if they have a significant influence on the values of other requirements. That will increase the penalty of ignoring requirements with positive influences on the values of selected requirements, as given by (\ref{eq_ch_dars_penalty}), resulting in lower overall value. This can be seen by comparing Figure~\ref{fig_ch_dars_ov_delta_dars_sbk} and Figure~\ref{fig_ch_dars_ev_delta_dars_sbk}. 

%
%To further clarify the conflicts amongst AV, EV, and OV, consider the following scenario. 
%
%let \gls{R}$=\{r_1,r_2,r_3\}$ be a requirement set with the estimated values $v_1=10,v_2=20,v_3=30$, costs $c_1=c_2=c_3$, and probabilities of being selected by users $p(r_1)=0.9,p(r_2)=0.9,p(r_3)=0.4$. We assume that the values of $r_2$ and $r_3$ highly depend on the presence of $r_1$ thus ignoring $r_1$ would significantly impact the values of $r_2$ and $r_3$ in a negative way. The following examples show the disadvantages of using AV (Example~\ref{ex_ch_dars_motivating_accumulated}) or EV (Example~\ref{ex_ch_dars_motivating_expected}) as the optimality criterion in requirement selection for $R$. \gls{v_i} and \gls{c_i} in these examples denote the estimated value and cost of a requirement \gls{r_i} respectively while \gls{p(r_i)} specifies the probability that $r_i$ is selected by users. 
%
%\begin{exmp}
%	\label{ex_ch_dars_motivating_accumulated}
%	Consider requirement selection for $R$ when budget is available only for one of the requirements $r_1$, $r_2$, or $r_3$. It is clear that when accumulated value (AV) is used as the optimality criterion, only $r_3$ with $v_3=30$ will be selected. As such, the value of $r_3$ may be negatively impacted, to a significant extent, by ignoring $r_1$ and this may result in value loss. Moreover, the accumulated value (AV) does not account for user preferences ignoring the fact that $r_3$ is less likely to be selected by users compared to $r_2$ ($p(r_3) < p(r_2)$). Ignoring user preferences may also result in value loss.
%\end{exmp}
%
%\begin{exmp}
%	\label{ex_ch_dars_motivating_expected}
%	Consider using expected value (EV) as the optimality criterion in Example~\ref{ex_ch_dars_motivating_accumulated}, where we have $E(v_1)=0.9 \times 10=9$, $E(v_2)=0.9 \times 20=18$, and $E(v_3)=0.4 \times 30=12$. \gls{E(v_i)} denote the expected value of a requirement $r_i$. It is clear that based on EV, requirement $r_2$ with the highest expected value will be selected. $r_1$ however will be ignored despite its significant impact on the value of $r_2$. Value loss hence may occur again as a result of ignoring $r_1$. Intuitively, users that would have used or purchased $r_2$ in the presence of $r_1$, now may change their minds in the absence of $r_1$. This cannot be captured by the selection methods that use expected value as the measure of optimality.
%\end{exmp}
%
%Example~\ref{ex_ch_dars_motivating_accumulated} and Example~\ref{ex_ch_dars_motivating_expected} show that the selection methods that use AV/EV as the optimality criterion may ignore highly influential requirements if they are of smaller estimated/expected values compared to other requirements. Overall value on th other hand, as presented in this thesis, captures value dependencies identified from user preferences. Hence, the penalties of ignoring (selecting) requirements with positive (negative) impacts on the value of the selected subset of requirements will be taken into account. 

\subsubsection{Mitigating the Value Loss} 

Ignoring value dependencies can pose a risk to the economic worth of software configurations and eventually result in value loss as given by (\ref{eq_ch_dars_penalty}). This risk can be be measured by the gap between the expected value of software and its overall value, which accounts for value dependencies, as depicted in Figure~\ref{fig_ch_dars_risk}. As shown in this figure, for each selection task performed at a specific price level, the gap between the expected value and the overall value of software configuration found by DARS was notably smaller than the gaps between the $\%$EV and $\%$OV provided by the PCBK method. Hence, using DARS contributed to a smaller risk of value loss in different configurations of software. 

\begin{figure*}[!htbp]
	\centering
	\hspace{0.0cm}\includegraphics[scale=0.6]{ch_dars/figs/result/fig_cs_risk}
	\caption{%
		Risk of value loss at different price levels. 
	}%
	\label{fig_ch_dars_risk}
\end{figure*}

We observed (Figure~\ref{fig_ch_dars_risk}) that the risk of value loss for the configurations found by DARS were under $5\%$ while this fluctuated from almost negligible to around $37\%$ in PCBK and SBK. In most configurations found by PCBK and SBK, an inconsistent pattern of ``the higher the price the higher the risk of value loss" was observed suggesting a higher risk for expensive configurations of software. The risk of value loss for the configurations found by the SBK method, however, converged to those found by DARS for $\%\text{Price} \geq 88$ as both methods chose more similar configurations (\protect\hyperlink{RQ1.4}{(\textbf{RQ1.4})}).

==> dars.tex <==
\chapter{The Integer Linear Programming Method (DARS-ILP) \protect \footnote{The main results of this chapter are presented in publications \protect\hyperlink{P1}{(\textbf{P1})}-\protect\hyperlink{P8}{(\textbf{P8})}.}}

% 4,6,7,8
\label{ch_dars}
\hypertarget{ch_dars}{ }
	
\input{ch_dars/introduction}
%\input{ch_dars/related}
\input{ch_dars/identification}
\input{ch_dars/modeling}
%------selection---------------------
\input{ch_dars/selection}
\input{ch_dars/selection_ov}
\input{ch_dars/selection_ilp}
\input{ch_dars/selection_blind}
%------validation---------------------
%\input{ch_dars/validation}
\input{ch_dars/case}
\input{ch_dars/case_description}
\input{ch_dars/case_identification}
\input{ch_dars/case_selection}
%\input{ch_dars/case_release}
\input{ch_dars/simulation}
\input{ch_dars/simulation_I}
\input{ch_dars/simulation_II}
\input{ch_dars/simulation_III}
\input{ch_dars/simulation_IV}
\input{ch_dars/simulation_V}
\input{ch_dars/simulation_VI}
%%------scalability---------------------
\input{ch_dars/scalability}
%%------conclusion---------------------
\input{ch_dars/conclusion}




==> lr1.tex <==
\begin{tabular}{|r|r|rrr|r|r|r|r|}
\hline
\textbf{Employed Model} &
  \textbf{Works} &
  \textbf{P1} &
  \textbf{P2} &
  \textbf{P3} &
  \textbf{P4} &
  \textbf{P5} &
  \textbf{P6} &
  \textbf{P7}
  \bigstrut\\
\hline
BKP &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\hline
\multirow{5}[10]{*}{BKP-PC} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\hline
Increase/Decrease_Value_Of (subsets of size 2) &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\hline
Increase/Decrease_Value_Of (subsets of any size) &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\hline
\end{tabular}%


==> rq_dars_ilp_case.tex <==
\begin{itemize}[leftmargin=1.5cm]
	\itemsep0em 
	\hypertarget{RQ1}{ }
	\item[(\textbf{RQ1})] How effective is DARS in considering value dependencies? 
	\hypertarget{RQ1.1}{ } 
	\item[(\textbf{RQ1.1})] How similar are the solutions found by DARS to those found by other selection methods?
	\hypertarget{RQ1.2}{ } 
	\item[(\textbf{RQ1.2})] What is the impact of using DARS on the overall value of software?  
	\hypertarget{RQ1.3}{ }
	\item[(\textbf{RQ1.3})] What is the relationship between maximizing the accumulated value, expected value, and overall value of a software product?
	\hypertarget{RQ1.4}{ }
	\item[(\textbf{RQ1.4})] How effective is DARS in mitigating value loss?
%	\item[(\textbf{RQ7})] What is the impact of using DARS-ILP on sales?  
%	\item[(\textbf{RQ8})] How effective is DARS-ILP in providing higher revenue for software products compared to the existing requirement selection methods?  
\end{itemize}

==> rq_dars_ip.tex <==
\begin{itemize}[leftmargin=1.8cm]
	\itemsep0em 
	\hypertarget{RQ1}{ }
	\item[(\textbf{RQ1})] What is the impact of using DARS-IP on the overall value of software products? 
	\hypertarget{RQ2}{ } 
	\item[(\textbf{RQ2})] What is the relationship between maximizing the accumulated value and overall value of software products?
	\hypertarget{RQ3}{ }
	\item[(\textbf{RQ3})] How effective is DARS-IP in mitigating the selection deficiency problem?
	\hypertarget{RQ4}{ }
	\item[(\textbf{RQ4})] What is the impact of value dependencies on the performance of DARS-IP? 
	\hypertarget{RQ5}{ }
	\item[(\textbf{RQ5})] How practical is DARS-IP for software projects?     
\end{itemize}

==> rq_dars_mip.tex <==
\begin{itemize}[leftmargin=1.8cm]
	\hypertarget{RQ10}{ }
	\item[(\textbf{RQ10})] How effective is the DARS-MLP method in reducing the value loss?
\end{itemize}

==> table_cs_dependencies.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\Huge
%\huge
%\LARGE
%\Large
%\large
%\normalsize (default)
%\small
%\footnotesize
%\scriptsize
%\tiny
\normalsize\rowcolors{1}{}{lightgray}
\resizebox {1\textwidth }{!}{
	\begin{tabular}{lrrl}
    \toprule[1.5pt]
\textbf{ID} &
\textbf{Value} &
\textbf{Cost} &
\textbf{\textit{Dependency Vector} $D_i = \{\sigma_{i,1}\rho_{i,1},...,\sigma_{i,26}\rho_{i,27}\}$}

\\ \midrule

$r_{1}$ &
$10$ &
$5$ &
$\{+0.00,+0.00,+0.00,+0.05,+0.05,+0.00,+0.60,+0.40,+0.00,+0.00,+0.00,+0.20,+0.00,+0.00,+0.00,+0.00,+0.40,+0.00,+0.00,+0.00,+0.05,+0.00,+0.00,+0.90,+0.00,+0.00,+0.00\}$
\\
$r_{2}$ &
$20$ &
$20$ &
$\{+1.00,+0.00,+0.00,+0.60,+0.10,+0.00,+0.60,+0.60,+0.10,+0.30,+0.30,+0.70,+0.00,+0.30,+0.00,+0.40,+0.40,+0.00,+0.00,+0.00,+0.10,+0.00,+0.20,+0.90,+0.00,+1.00,+0.00\}$
\\
$r_{3}$ &
$4$ &
$0$ &
$\{+1.00,+0.00,+0.00,+0.50,+0.10,+0.00,+0.60,+0.00,+0.00,+0.00,+0.00,+0.20,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{4}$ &
$17$ &
$10$ &
$\{+0.00,+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.40,+0.00,+0.00,+0.20,+0.00,+0.40,+0.00,+0.00,+0.00,+0.00,+0.10,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{5}$ &
$3$ &
$1$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.10,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{6}$ &
$20$ &
$20$ &
$\{+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.60,+0.00,+0.30,+0.30,+0.40,+0.00,+0.00,+0.00,+0.00,+0.40,+0.40,+0.00,+0.00,+0.00,+0.00,+0.00,+0.30,+0.90,+0.00,+1.00,+0.00\}$
\\
$r_{7}$ &
$15$ &
$6$ &
$\{+0.60,+0.60,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.60,+0.00,+0.00,+0.00\}$
\\
$r_{8}$ &
$9$ &
$5$ &
$\{+1.00,+0.80,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+1.00,+0.00,+0.00\}$
\\
$r_{9}$ &
$20$ &
$16$ &
$\{+0.00,+0.50,+0.00,+0.00,+0.00,+1.00,+0.00,+0.30,+0.00,+0.00,+0.80,+0.20,+0.30,+0.00,+0.05,+0.40,+0.00,+0.00,+0.00,+0.00,+0.05,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{10}$ &
$16$ &
$10$ &
$\{+0.00,+0.70,+0.00,+0.00,+0.05,+0.70,+0.00,+0.30,+0.00,+0.00,+0.00,+0.00,+0.40,+0.00,+0.00,+0.20,+0.00,+0.00,+0.00,+0.00,+0.10,+0.60,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{11}$ &
$20$ &
$4$ &
$\{+0.00,+0.00,+0.00,+0.40,+0.00,+0.50,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,-0.05,+0.00,+0.00,+0.00,+0.05,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{12}$ &
$10$ &
$3$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.10,+0.40,+0.00,+0.00,+0.00,+0.00,+0.00,+0.40,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{13}$ &
$6$ &
$5$ &
$\{+0.00,+0.00,+0.00,+0.00,+0.00,+1.00,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.10,+0.40,+0.00,+0.00,+0.00,+0.00,+0.00,+0.60,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{14}$ &
$8$ &
$7$ &
$\{+1.00,+0.60,+0.00,+0.00,+0.00,+0.90,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{15}$ &
$8$ &
$15$ &
$\{+0.00,+1.00,+0.00,+0.00,+0.00,+0.50,+0.00,+0.00,+0.00,+0.00,+0.20,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{16}$ &
$10$ &
$13$ &
$\{+0.00,+1.00,+0.00,+0.00,+0.00,+0.50,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.00,+0.50,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,-0.02,-0.10\}$
\\
$r_{17}$ &
$6$ &
$14$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.20,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,-0.05,-0.05\}$
\\
$r_{18}$ &
$10$ &
$3$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{19}$ &
$20$ &
$10$ &
$\{+0.00,+1.00,+0.00,+0.70,+0.50,+1.00,+0.00,+0.50,+1.00,+0.60,+0.40,+0.00,+0.00,+0.10,+0.80,+0.80,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{20}$ &
$20$ &
$7$ &
$\{+0.00,+1.00,+0.00,+0.70,+0.50,+1.00,+0.60,+0.50,+1.00,+0.60,+0.40,+0.00,+0.00,+0.10,+0.80,+0.80,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{21}$ &
$15$ &
$12$ &
$\{+0.00,+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00,+0.00,+0.30,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{22}$ &
$20$ &
$15$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.10,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.10,+0.00,+0.00\}$
\\
$r_{23}$ &
$20$ &
$8$ &
$\{+0.00,+1.00,+0.00,+0.00,+0.00,+0.30,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{24}$ &
$5$ &
$2$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.10,+0.10,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,-0.01,+0.00,+0.00\}$
\\
$r_{25}$ &
$0$ &
$10$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.80,+0.00,+0.00,+0.00,+0.00\}$
\\
$r_{26}$ &
$0$ &
$0$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+1.00\}$
\\
$r_{27}$ &
$0$ &
$1$ &
$\{+1.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00,+0.00\}$
\\
$\textbf{Sum}$ &
$\textbf{312}$ &
$\textbf{222}$ &
$$
\\
\bottomrule[1.5pt]
\end{tabular}}%


==> table_cs_dependencies_1.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\normalsize\rowcolors{1}{}{lightgray}
\huge\resizebox {1.1\textwidth }{!}{
	\begin{tabular}{lrrlllllllllllllllllllllllllll}
	\toprule[1.5pt]
	\textbf{ID} &
	\textbf{Value} &
	\textbf{Cost} &
	\multicolumn{27}{l}{\boldmath{}\textbf{\textbf{Dependency Vector} $D_i=\{\sigma_{i,1}\rho_{i,1},...,\sigma_{i,27}\rho_{i,27}\}$}\unboldmath{}}
	\\ \midrule
	$r_{1}$ &
	$10$ &
	$5$ &
	$\{\pm 0.00$ ,&
		$\pm 0.00$, &
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.05$ ,&
		\cellcolor{gray!25}$+0.05$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.20$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.05$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.90$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{2}$ &
	$20$ &
	$20$ &
	$\{+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		\cellcolor{gray!25}$+0.70$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.20$ ,&
		\cellcolor{gray!25}$+0.90$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{3}$ &
	$4$ &
	$0$ &
	$\{+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.50$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.20$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{4}$ &
	$17$ &
	$10$ &
	$\{\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.20$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{5}$ &
	$3$ &
	$1$ &
	$\{+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{6}$ &
	$20$ &
	$20$ &
	$\{\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		\cellcolor{gray!25}$+0.90$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{7}$ &
	$15$ &
	$6$ &
	$\{+0.60$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{8}$ &
	9 &
	5 &
	$\{+1.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{9}$ &
	20 &
	16 &
	$\{\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.50$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		\cellcolor{gray!25}$+0.20$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.05$,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		0.05 ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{10}$ &
	16 &
	10 &
	$\{\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.70$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.05$ ,&
		\cellcolor{gray!25}$+0.70$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.30$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.20$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{11}$ &
	20 &
	4 &
	$\{\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.50$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!55}$-0.05$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.05$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{12}$ &
	10 &
	3 &
	$\{+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{13}$ &
	6 &
	5 &
	$\{\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.10$ ,&
		\cellcolor{gray!25}$+0.40$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{14}$ &
	8 &
	7 &
	$\{+1.00$ ,&
		\cellcolor{gray!25}$+0.60$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.90$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{15}$ &
	8 &
	15 &
	$\{\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.50$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.20$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00\}$
	\\
	$r_{16}$ &
	10 &
	13 &
	$\{\pm 0.00$ ,&
		\cellcolor{gray!25}$+1.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.50$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.80$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!25}$+0.50$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		$\pm 0.00$ ,&
		\cellcolor{gray!55}$-0.02$ ,&
		\cellcolor{gray!55}$-0.10\}$
		\\
		$r_{17}$ &
		6 &
		14 &
		$\{+1.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			\cellcolor{gray!25}$+0.80$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			\cellcolor{gray!25}$+0.20$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			$\pm 0.00$ ,&
			\cellcolor{gray!55}$-0.05$ ,&
			\cellcolor{gray!55}$-0.05\}$
			\\
			$r_{18}$ &
			10 &
			3 &
			$\{+1.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00\}$
			\\
			$r_{19}$ &
			20 &
			10 &
			$\{\pm 0.00$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				$\pm 0.00$ ,&
				\cellcolor{gray!25}$+0.70$ ,&
				\cellcolor{gray!25}$+0.50$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				$\pm 0.00$ ,&
				\cellcolor{gray!25}$+0.50$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				\cellcolor{gray!25}$+0.60$ ,&
				\cellcolor{gray!25}$+0.40$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				\cellcolor{gray!25}$+0.10$ ,&
				\cellcolor{gray!25}$+0.80$ ,&
				\cellcolor{gray!25}$+0.80$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				\cellcolor{gray!25}$+0.80$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00\}$
			\\
			$r_{20}$ &
			20 &
			7 &
			$\{\pm 0.00$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.70$ ,&
				\cellcolor{gray!25}$+0.50$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				\cellcolor{gray!25}$+0.60$ ,&
				\cellcolor{gray!25}$+0.50$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				\cellcolor{gray!25}$+0.60$ ,&
				\cellcolor{gray!25}$+0.40$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.10$ ,&
				\cellcolor{gray!25}$+0.80$ ,&
				\cellcolor{gray!25}$+0.80$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.80$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00\}$
			\\
			$r_{21}$ &
			15 &
			12 &
			$\{\pm 0.00$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.80$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.80$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.30$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00\}$
			\\
			$r_{22}$ &
			20 &
			15 &
			$\{+1.00$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.10$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.10$ ,&
				$\pm 0.00$,&
				$\pm 0.00\}$
			\\
			$r_{23}$ &
			20 &
			8 &
			$\{\pm 0.00$ ,&
				\cellcolor{gray!25}$+1.00$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.30$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00\}$
			\\
			$r_{24}$ &
			5 &
			2 &
			$\{+1.00$ &
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				\cellcolor{gray!25}$+0.10$ ,&
				\cellcolor{gray!25}$+0.10$ ,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00$ ,&
				\cellcolor{gray!55}$-0.01$ ,&
				$\pm 0.00$ ,&
				$\pm 0.00\}$
			\\
			$r_{25}$ &
			$0$ &
			$10$ &
			$\{+1.00$ &
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				\cellcolor{gray!25}$+0.80$ ,&
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00$ ,& 
				$\pm 0.00\}$
			\\
			$r_{26}$ &
			$0$ & 
			$0$  &
			$\{+1.00$ ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00\}$
			\\
			$r_{27}$ &
			$0$  &
			$1$ &
			$\{+1.00$ ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00$  ,&
				$\pm 0.00\}$
				\\ \midrule
				$\textbf{Sum}$ &
				$\textbf{312}$ &
				$\textbf{222}$ &
				$$
			\\	\toprule[1.5pt]
		\end{tabular}}%


==> table_cs_solutions.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\rowcolors{1}{}{lightgray}
\resizebox {0.8\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'Sheet6'
	\begin{tabular}{llll}
		\toprule[1.5pt]
		\textbf{Budget (relative)} &
		\textbf{Selection Model} &
		\textbf{Overall Value (percent)} &
		\boldmath{}\textbf{Solution Vector ($r_1,...,r_{23}$)}\unboldmath{}
		\\ \midrule[1.5pt]
		\multirow{3}[1]{*}{16} &
		BKP &
		5.21 &
		$\{0,1,1,0,0,0,0,0,0,0,1,0,0,0,0,1,0,0,0,0,0,0,0\}$
		\\
		&
		BKP-PC &
		10.74 &
		$\{0,0,0,0,0,0,1,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,1\}$
		\\
		&
		GORS &
		12.88 &
		$\{0,0,0,0,0,0,1,0,0,0,1,0,0,0,0,1,0,1,0,0,0,0,0\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{46} &
		BKP &
		23.25 &
		$\{1,1,1,0,0,0,1,0,0,0,1,0,0,0,0,1,0,1,0,0,0,0,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		19.94 &
		$\{0,0,0,0,0,0,1,0,0,0,0,0,0,0,0,0,0,1,0,0,0,1,1\}$
		\\
		&
		GORS &
		26.63 &
		$\{0,0,0,0,0,0,1,0,0,0,1,0,1,0,0,1,0,1,0,0,0,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{71} &
		BKP &
		31.07 &
		$\{1,1,1,1,0,0,1,0,0,1,1,1,0,0,0,1,0,1,0,0,0,0,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		19.94 &
		$\{0,0,0,0,0,0,1,0,0,0,0,0,0,0,0,0,0,1,0,0,0,1,1\}$
		\\
		&
		GORS &
		34.60 &
		$\{1,1,1,0,0,0,1,0,0,0,1,1,1,0,0,1,0,1,0,0,0,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{76} &
		BKP &
		32.06 &
		$\{1,1,1,1,0,0,1,0,0,1,1,1,1,0,0,1,0,1,0,0,0,0,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		19.94 &
		$\{0,0,0,0,0,0,1,0,0,0,0,0,0,0,0,0,0,1,0,0,0,1,1\}$
		\\
		&
		GORS &
		35.74 &
		$\{1,1,1,1,0,0,1,0,0,0,1,1,0,0,0,1,0,1,0,0,0,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{81} &
		BKP &
		31.90 &
		$\{1,1,1,1,0,0,1,0,0,1,1,0,1,0,0,1,1,1,0,0,0,0,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		19.94 &
		$\{0,0,0,0,0,0,1,0,0,0,0,0,0,0,0,0,0,1,0,0,0,1,1\}$
		\\
		&
		GORS &
		37.98 &
		$\{0,0,0,1,0,0,0,0,0,0,1,0,0,1,0,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{141} &
		BKP &
		44.11 &
		$\{1,1,1,1,0,0,1,0,1,1,1,1,1,0,0,1,1,1,0,1,0,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		59.45 &
		$\{1,1,1,1,0,0,1,0,0,1,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{146} &
		BKP &
		45.40 &
		$\{1,1,1,1,0,0,1,0,1,1,1,1,0,0,0,1,1,1,0,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		60.43 &
		$\{1,1,1,1,0,0,1,1,0,0,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{151} &
		BKP &
		46.87 &
		$\{1,1,1,1,0,0,1,0,1,1,1,1,1,0,0,1,1,1,0,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		62.27 &
		$\{1,1,1,1,0,1,1,0,0,0,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{156} &
		BKP &
		46.87 &
		$\{1,1,1,1,0,0,1,0,1,1,1,1,1,0,0,1,1,1,0,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		62.27 &
		$\{1,1,1,1,0,1,1,0,0,0,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{161} &
		BKP &
		50.12 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,1,0,0,1,1,1,0,1,0,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		64.23 &
		$\{1,1,1,1,0,1,1,0,0,1,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{166} &
		BKP &
		51.41 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,0,0,0,1,1,1,0,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		64.72 &
		$\{1,1,1,1,0,1,1,0,1,0,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{171} &
		BKP &
		52.88 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,1,0,0,1,1,1,0,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		64.72 &
		$\{1,1,1,1,0,1,1,0,1,0,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{176} &
		BKP &
		52.88 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,1,0,0,1,1,1,0,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		66.69 &
		$\{1,1,1,1,0,1,1,1,0,1,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{181} &
		BKP &
		51.35 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,1,0,0,1,1,1,1,1,0,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		67.18 &
		$\{1,1,1,1,0,1,1,1,1,0,1,1,1,1,1,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{186} &
		BKP &
		52.64 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,0,0,0,1,1,1,1,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		73.83 &
		$\{1,1,0,1,1,1,1,1,1,1,1,1,1,1,0,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{191} &
		BKP &
		54.11 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,1,0,0,1,1,1,1,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		75.31 &
		$\{1,1,1,1,1,1,1,1,1,1,1,1,1,1,0,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[2]{*}{196} &
		BKP &
		54.11 &
		$\{1,1,1,1,0,1,1,0,1,1,1,1,1,0,0,1,1,1,1,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		53.37 &
		$\{0,0,0,1,1,0,1,1,0,0,1,0,1,1,1,1,1,1,0,0,1,1,1\}$
		\\
		&
		GORS &
		75.31 &
		$\{1,1,1,1,1,1,1,1,1,1,1,1,1,1,0,1,1,1,0,0,1,1,1\}$
		\bigstrut[b]\\
		\hline
		\multirow{3}[1]{*}{246} &
		BKP &
		100.00 &
		$\{1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1\}$
		\bigstrut[t]\\
		&
		BKP-PC &
		100.00 &
		$\{1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1\}$
		\\
		&
		GORS &
		100.00 &
		$\{1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1,1\}$
		\\ \bottomrule[1.5pt]
	\end{tabular}}%


==> table_data.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\resizebox {0.7\textwidth}{!}{
\begin{tabular}{| r | r | r | r |  r| r |  r | r | r | r | r | r | r | r | r | r |}
\Xhline{4\arrayrulewidth}
 &
  Requirement &
  $r_0$ &
  $r_1$ &
  $r_2$ &
  $r_3$ &
  $r_4$ &
  $r_5$ &
  $r_6$ &
  $r_7$ &
  $r_8$ &
  $r_9$ &
  $r_{10}$ &
  $r_{11}$ &
  $r_{12}$ &
  $r_{13}$
  \bigstrut\\
\hline
\multirow{2}[4]{*}{\textbf{RAN}} &
  Value &
  $12$ &
  $6$ &
  $5$ &
  $7$ &
  $12$ &
  $16$ &
  $3$ &
  $3$ &
  $4$ &
  $5$ &
  $1$ &
  $1$ &
  $21$ &
  $3$
  \bigstrut\\
\cline{2-16} &
  Cost &
  $1$ &
  $2$ &
  $3$ &
  $4$ &
  $6$ &
  $11$ &
  $4$ &
  $6$ &
  $7$ &
  $12$ &
  $4$ &
  $6$ &
  $23$ &
  $10$
  \bigstrut\\
\hline
\multirow{2}[4]{*}{\textbf{PMR}} &
  Value &
  $0$ &
  $6$ &
  $3$ &
  $11$ &
  $32$ &
  $20$ &
  $9$ &
  $4$ &
  $25$ &
  $9$ &
  $3$ &
  $\--$ &
  $\--$ &
  $\--$ 
  \bigstrut\\
\cline{2-16} &
  Cost &
  $6$ &
  $5$ &
  $6$ &
  $19$ &
  $28$ &
  $4$ &
  $5$ &
  $7$ &
  $10$ &
  $3$ &
  $8$ &
  $\--$ &
  $\--$ &
  $\--$ 
  \bigstrut\\
\Xhline{4\arrayrulewidth}
\end{tabular}
}%



==> table_ex_all.tex <==
%\rowcolor{lightgray}
\rowcolors{1}{}{lightgray}
\resizebox {0.7\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'allsolution_requirements_0.125'
% Table generated by Excel2LaTeX from sheet 'allsolution_requirements_0.125'
% Table generated by Excel2LaTeX from sheet 'allsolution_requirements_0.125'
% Table generated by Excel2LaTeX from sheet 'allsolution_requirements_0.125'
\begin{tabular}{llccc}
	\toprule[1.5pt]
	$X_k=$$\{ x_{0},x_{1},x_{2},x_{3} \}$ &
	$P_k=$$\{ p_{0},p_{1},p_{2},p_{3} \}$ &
	$AC=\displaystyle \sum_{i=1}^{n} x_i c_i$ &
	$ACV=\displaystyle \sum_{i=1}^{n} x_iv_i$ &
	$OCV=\displaystyle \sum_{i=1}^{n} x_i (v_i - p_iv_i)$
	\\ \midrule
	$X_{0}=\{0,0,0,0\}$ &
	$P_{0}=\{0.0,0.0,0.0,0.0\}$ &
	$0.0$ &
	$0.0$ &
	$0.0$
	\\
	$X_{1}=\{1,0,0,0\}$ &
	$P_{1}=\{0.7,0.0,0.0,0.0\}$ &
	$10.0$ &
	$20.0$ &
	$6.0$
	\\
	$X_{2}=\{0,1,0,0\}$ &
	$P_{2}=\{0.0,0.3,0.0,0.0\}$ &
	$10.0$ &
	$10.0$ &
	$7.0$
	\\
	$X_{3}=\{1,1,0,0\}$ &
	$P_{3}=\{0.7,0.3,0.0,0.0\}$ &
	$20.0$ &
	$30.0$ &
	$13.0$
	\\
	$X_{4}=\{0,0,1,0\}$ &
	$P_{4}=\{0.0,0.0,0.7,0.0\}$ &
	$15.0$ &
	$50.0$ &
	$15.0$
	\\
	$X_{5}=\{1,0,1,0\}$ &
	$P_{5}=\{0.7,0.0,0.7,0.0\}$ &
	$25.0$ &
	$70.0$ &
	$21.0$
	\\
	$X_{6}=\{0,1,1,0\}$ &
	$P_{6}=\{0.0,0.3,0.7,0.0\}$ &
	$25.0$ &
	$60.0$ &
	$22.0$
	\\
	$X_{7}=\{1,1,1,0\}$ &
	$P_{7}=\{0.7,0.3,0.7,0.0\}$ &
	$35.0$ &
	$80.0$ &
	$28.0$
	\\
	$X_{8}=\{0,0,0,1\}$ &
	$P_{8}=\{0.0,0.0,0.0,0.2\}$ &
	$10.0$ &
	$10.0$ &
	$8.0$
	\\
	$X_{9}=\{1,0,0,1\}$ &
	$P_{9}=\{0.7,0.0,0.0,0.2\}$ &
	$20.0$ &
	$30.0$ &
	$14.0$
	\\
	$X_{10}=\{0,1,0,1\}$ &
	$P_{10}=\{0.0,0.2,0.0,0.2\}$ &
	$20.0$ &
	$20.0$ &
	$16.0$
	\\
	$X_{11}=\{1,1,0,1\}$ &
	$P_{11}=\{0.7,0.2,0.0,0.2\}$ &
	$30.0$ &
	$40.0$ &
	$22.0$
	\\
	$X_{12}=\{0,0,1,1\}$ &
	$P_{12}=\{0.0,0.0,0.6,0.2\}$ &
	$25.0$ &
	$60.0$ &
	$28.0$
	\\
	$X_{13}=\{1,0,1,1\}$ &
	$P_{13}=\{0.5,0.0,0.5,0.2\}$ &
	$35.0$ &
	$80.0$ &
	$43.0$
	\\
	$X_{14}=\{0,1,1,1\}$ &
	$P_{14}=\{0.0,0.2,0.6,0.2\}$ &
	$35.0$ &
	$70.0$ &
	$36.0$
	\\
	$X_{15}=\{1,1,1,1\}$ &
	$P_{15}=\{0.0,0.0,0.0,0.0\}$ &
	$45.0$ &
	$90.0$ &
	$90.0$
	\\ \bottomrule[1.5pt]
\end{tabular}
}





==> table_ex_all_2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet5'
\resizebox {1\textwidth }{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
	\Xhline{4\arrayrulewidth}
$\textbf{Solution}$ &
  $S_0$ &
  $S_1$ &
  $S_2$ &
  $S_3$ &
  $S_4$ &
  $S_5$ &
  $S_6$ &
  $S_7$ &
  $S_8$ &
  $S_9$ &
  $S_{10}$ &
  $S_{11}$ &
  $S_{12}$ &
  $S_{13}$ &
  $S_{14}$ &
  $S_{15}$
  \bigstrut\\
\hline
$\textbf{O}$ &
  $\{\}$ &
  $\{r_1\}$ &
  $\{r_2\}$ &
  $\{r_3\}$ &
  $\{r_4\}$ &
  $\{r1_,r_2\}$ &
  $\{r_1,r_3\}$ &
  $\{r_2,r_4\}$ &
  $\{r_2,r_3\}$ &
  $\{r_2,r_4\}$ &
  $\{r_3,r_4\}$ &
  $\{r_1,r_2,r_3\}$ &
  $\{r_1,r_2,r_4\}$ &
  $\{r_1,r_3,r_4\}$ &
  $\{r_2,r_3,r_4\}$ &
  $\{r_1,r_2,r_3,r_4\}$
  \bigstrut\\
\hline
$\tilde{\textbf{O}}$ &
  $\{r_1,r_2,r_3,r_4\}$ &
  $\{r_2,r_3,r_4\}$ &
	$\{r_1,r_3,r_4\}$ &
  $\{r_1,r_2,r_4\}$ &
  $\{r_1,r_2,r_3\}$ &
  $\{r_3,r_4\}$ &
  $\{r_2,r_4\}$ &
  $\{r_2,r_3\}$ &
  $\{r_2,r_4\}$ &
  $\{r_1,r_3\}$ &
  $\{r1_,r_2\}$ &
  $\{r_4\}$ &
  $\{r_3\}$ &
  $\{r_2\}$ &
  $\{r_1\}$ &
	$\{\}$ 

  \bigstrut\\
\hline
$\textbf{AC}$ &
  $0$ &
  $10$ &
  $10$ &
  $15$ &
  $10$ &
  $20$ &
  $25$ &
  $20$ &
  $25$ &
  $20$ &
  $25$ &
  $35$ &
  $30$ &
  $35$ &
  $35$ &
  $45$
  \bigstrut\\
\hline
$\textbf{AV}$ &
  $0$ &
  $20$ &
  $10$ &
  $50$ &
  $10$ &
  $30$ &
  $70$ &
  $30$ &
  $60$ &
  $20$ &
  $60$ &
  $80$ &
  $40$ &
  $80$ &
  $70$ &
  $90$
  \bigstrut\\
\hline
$\textbf{OV}$ &
  $0$ &
  $4$ &
  $8$ &
  $15$ &
  $8$ &
  $12$ &
  $21$ &
  $12$ &
  $23$ &
  $16$ &
  $23$ &
  $29$ &
  $20$ &
  $36$ &
  $31$ &
	$90$ 
  \bigstrut\\
	\Xhline{4\arrayrulewidth}
\end{tabular}}

==> table_ex_constraints.tex <==
\rowcolors{1}{}{lightgray}
\resizebox {0.4\textwidth }{!}{\begin{tabular}{ccccccccc}
  \toprule[1.5pt]
  \head{} & \head{$x_1$} & \head{$x_2$} & \head{$x_3$} & \head{$x_4$} & \head{$1-x_1$} & \head{$1-x_2$} & \head{$1-x_3$} & \head{$1-x_4$} \\
  %\midrule
	\Xhline{3\arrayrulewidth}
  $x_1$ & $-$ & $\leq$ & $\leq$ & $\leq$ &  $-$ & $\leq$ & $\leq$ & $\leq$ \\
  $x_2$ & $\leq$ & $-$ & $\leq$ & $\leq$ &  $-$ & $-$ & $-$ & $-$ \\
  $x_3$ & $\leq$ & $\leq$ & $-$ & $\leq$ &  $-$ & $-$ & $-$ & $\leq$ \\
  $x_4$ & $-$ & $\leq$ & $\leq$ & $-$    &  $-$ & $-$ & $-$ & $-$ \\

  \bottomrule[1.5pt]
\end{tabular}}



==> table_ex_overall_influence.tex <==
\rowcolors{1}{}{lightgray}
\resizebox {0.9\textwidth }{!}{\begin{tabular}{cccccc}
  \toprule[1.5pt]
  \head{$OI_{i,j}=\rho_{i,j}^{+\infty}-\rho_{i,j}^{-\infty}$} & \head{$r_1$} & \head{$r_2$} & \head{$r_3$} & \head{$r_4$} & \head{$r_5$}\\
  %\midrule
	\Xhline{3\arrayrulewidth}
  $r_1$ & $0.0-0.0=0.0$ & $0.4-0.0=0.0$ & $0.2-0.3=-0.1$ & $0.3-0.0=0.3$ & $0.0-0.5=-0.5$\\
  $r_2$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.2-0.0=0.2$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ \\
  $r_3$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ \\
  $r_4$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ \\
  $r_5$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ & $0.0-0.0=0.0$ \\
  \bottomrule[1.5pt]
\end{tabular}}



==> table_ex_overall_strengths.tex <==
\rowcolors{1}{}{lightgray}
\resizebox {0.7\textwidth }{!}{\begin{tabular}{cccccc}
  \toprule[1.5pt]
  \head{$OI_{i,j}=\rho_{i,j}^{+\infty}-\rho_{i,j}^{-\infty}$} & \head{$r_1$} & \head{$r_2$} & \head{$r_3$} & \head{$r_4$} & \head{$r_5$}\\
  %\midrule
	\Xhline{3\arrayrulewidth}
  $r_1$ & $0.0/0.0$ & $0.4/0.0$ & $0.2/0.3$ & $0.3/0.0$ & $0.0/0.5$\\
  $r_2$ & $0.0/0.0$ & $0.0/0.0$ & $0.2/0.0$ & $0.0/0.0$ & $0.0/0.0$ \\
  $r_3$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ & $0.0$ & $0.0/0.0$ \\
  $r_4$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ \\
  $r_5$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ & $0.0/0.0$ \\
  \bottomrule[1.5pt]
\end{tabular}}



==> table_lr.tex <==
\LARGE
%\rowcolors{1}{}{lightmyblue}
\resizebox {0.8\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'Sheet1'
% Table generated by Excel2LaTeX from sheet 'Sheet1'
% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{tabular}{l|l|lllllll}
	\toprule[1.5pt]
	\textbf{\cellcolor{header}\textcolor{white}{Employed Model}}&
	\textbf{\cellcolor{header}\textcolor{white}{Works from the Literature}} &
	\textbf{\cellcolor{header}\textcolor{white}{P1}} &
	\textbf{\cellcolor{header}\textcolor{white}{P2}} &
	\textbf{\cellcolor{header}\textcolor{white}{P3}} &
	\textbf{\cellcolor{header}\textcolor{white}{P4}} &
	\textbf{\cellcolor{header}\textcolor{white}{P5}} &
	\textbf{\cellcolor{header}\textcolor{white}{P6}} &
	\textbf{\cellcolor{header}\textcolor{white}{P7}}
	\\\midrule[1.5pt]
	\multicolumn{1}{l|}{\cellcolor{myblue!30}BKP} 
	\cellcolor{myblue!30}&\begin{tabular}[t]{@{}c@{}} \cite{karlsson_optimizing_1997,jung_optimizing_1998,zhang_multi_objective_2007,baker_search_2006,finkelstein2009search,zhang2011comparing,del2010ant,kumari2012software} \phantom{sssssssssssss} \end{tabular} &
	\cellcolor{myblue!30}NO &
	\cellcolor{myblue!30}NO &
	\cellcolor{myblue!30}NO &
	\cellcolor{myblue!30}NO &
	\cellcolor{myblue!30}NO &
	\cellcolor{myblue!30}NO &
	\cellcolor{myblue!30}NO
	\\ 
	\multicolumn{1}{l|}{\cellcolor{myblue!20}BKP-PC} &
	{1}\cellcolor{myblue!20}\begin{tabular}[t]{@{}c@{}} \cite{veerapen2015integer,brasil_multiobjective_2012,bagnall_next_2001,greer_software_2004,boschetti_lagrangian_2014,ruhe_quantitative_2003,van2011quantitative,zhang2010search,tonella2010using,freitas2011software}\\\cite{colares_new_2009,saliu2007bi,saliu2005supporting,jiang2010hybrid,van2005determination,ngo2009optimized,chen2013ant,del2011requirements,araujo2016architecture,colares2009new,pitangueira2016risk}\end{tabular}  &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}NO
	\\
	\multicolumn{1}{l|}{\cellcolor{myblue!20}} &
	\cellcolor{myblue!20}\cite{van2008software,ngo_wicked_2008} &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}NO
	\\
	\multicolumn{1}{l|}{\cellcolor{myblue!20}} &
	\cellcolor{myblue!20}\cite{tonella2013interactive,xuan2012solving,saliu2005software} &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}NO
	\\
	\multicolumn{1}{l|}{\cellcolor{myblue!20}} &
	\cellcolor{myblue!20}\cite{li2016value} &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}NO &
	\cellcolor{myblue!20}YES &
	\cellcolor{myblue!20}NO
	\\
	\multicolumn{1}{l|}{\cellcolor{myblue!10}Increase/Decrease\_Value\_Of} &
	\cellcolor{myblue!10}\cite{li_integrated_2010,sagrado_multi_objective_2013,Zhang_RIM_2013} (Subsets of Size 2)&
	\cellcolor{myblue!10}YES &
	\cellcolor{myblue!10}NO &
	\cellcolor{myblue!10}YES &
	\cellcolor{myblue!10}YES &
	\cellcolor{myblue!10}NO &
	\cellcolor{myblue!10}YES &
	\cellcolor{myblue!10}YES
	\\
	\multicolumn{1}{l|}{\cellcolor{myblue!10}} &
	\cellcolor{myblue!10}\cite{van_den_akker_flexible_2005} (Subsets of Any Size)&
	\cellcolor{myblue!10}YES &
	\cellcolor{myblue!10}YES &
	\cellcolor{myblue!10}NO &
	\cellcolor{myblue!10}NO &
	\cellcolor{myblue!10}NO &
	\cellcolor{myblue!10}YES &
	\cellcolor{myblue!10}YES
	\\\bottomrule[1.5pt]
\end{tabular}
}




==> table_lr1.tex <==
\LARGE
%\rowcolors{1}{}{lightmyblue}
\resizebox {0.9\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'Sheet1'
	% Table generated by Excel2LaTeX from sheet 'Sheet1'
	% Table generated by Excel2LaTeX from sheet 'Sheet4'
	% Table generated by Excel2LaTeX from sheet 'Sheet1'
	\begin{tabular}{l|l|lllllll}
		\hline
		\textbf{\cellcolor{header}\textcolor{white}{Employed Model}} &
		\textbf{\cellcolor{header}\textcolor{white}{Works}} &
		\textbf{\cellcolor{header}\textcolor{white}{P1}} &
		\textbf{\cellcolor{header}\textcolor{white}{P2}} &
		\textbf{\cellcolor{header}\textcolor{white}{P3}} &
		\textbf{\cellcolor{header}\textcolor{white}{P4}} &
		\textbf{\cellcolor{header}\textcolor{white}{P5}} &
		\textbf{\cellcolor{header}\textcolor{white}{P6}} &
		\textbf{\cellcolor{header}\textcolor{white}{P7}}
		\bigstrut\\
		\hline
		\cellcolor{myblue!30} BKP & 
		\cellcolor{myblue!30}\begin{tabular}[t]{@{}c@{}} \cite{karlsson_optimizing_1997,jung_optimizing_1998,zhang_multi_objective_2007,baker_search_2006,finkelstein2009search,zhang2011comparing,del2010ant,kumari2012software} \phantom{sssssssssssss} \end{tabular}&
		\cellcolor{myblue!30}NO &
		\cellcolor{myblue!30}NO &
		\cellcolor{myblue!30}NO &
		\cellcolor{myblue!30}NO &
		\cellcolor{myblue!30}NO &
		\cellcolor{myblue!30}NO &
		\cellcolor{myblue!30}NO
		
		\bigstrut\\
		\hline
		\multirow{4}[10]{*}{BKP-PC} &
		\cellcolor{myblue!20}\begin{tabular}[t]{@{}c@{}} \cite{veerapen2015integer,brasil_multiobjective_2012,sagrado_multi_objective_2013,bagnall_next_2001,greer_software_2004,boschetti_lagrangian_2014,ruhe_quantitative_2003,van2011quantitative,zhang2010search,tonella2010using,freitas2011software}\\ \cellcolor{myblue!20}\cite{colares_new_2009,saliu2007bi,saliu2005supporting,jiang2010hybrid,van2005determination,ngo2009optimized,chen2013ant,del2011requirements,araujo2016architecture,colares2009new,pitangueira2016risk}\end{tabular}  &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}NO  &
		\cellcolor{myblue!20}NO  &
		\cellcolor{myblue!20}NO  &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}NO
		
		\bigstrut\\
		\cline{2-9}  & 
		
		\cellcolor{myblue!20}\cite{van2008software,ngo_wicked_2008} &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}NO
		
		\bigstrut\\
		\cline{2-9} & 
		
		\cellcolor{myblue!20}\cite{tonella2013interactive,xuan2012solving,saliu2005software} &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}NO
		
		\bigstrut\\
		\cline{2-9} & 
		
		\cellcolor{myblue!20}\cite{li2016value} &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}NO &
		\cellcolor{myblue!20}YES &
		\cellcolor{myblue!20}NO
		
		\bigstrut\\
		\hline
		
		\cellcolor{myblue!10} Increase/Decrease\_Value\_Of (subsets of size 2) &
		\cellcolor{myblue!10}\cite{li_integrated_2010,sagrado_multi_objective_2013,Zhang_RIM_2013}&
		\cellcolor{myblue!10}YES &
		\cellcolor{myblue!10}NO &
		\cellcolor{myblue!10}YES &
		\cellcolor{myblue!10}YES &
		\cellcolor{myblue!10}NO &
		\cellcolor{myblue!10}YES &
		\cellcolor{myblue!10}YES
		
		\bigstrut\\
		\hline
		
		\cellcolor{myblue!10} Increase/Decrease\_Value\_Of (subsets of any size) &
		\cellcolor{myblue!10}\cite{van_den_akker_flexible_2005}&
		\cellcolor{myblue!10}YES &
		\cellcolor{myblue!10}YES &
		\cellcolor{myblue!10}NO &
		\cellcolor{myblue!10}NO &
		\cellcolor{myblue!10}NO &
		\cellcolor{myblue!10}YES &
		\cellcolor{myblue!10}YES
		\\\bottomrule[1.5pt]
		
	\end{tabular}%
}



==> table_lr2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{tabular}{|l|l|lllllll|}
\hline
\textbf{\cellcolor{header}\textcolor{white}{Employed Model}} &
  \textbf{\cellcolor{header}\textcolor{white}{Works}} &
  \textbf{\cellcolor{header}\textcolor{white}{P1}} &
  \textbf{\cellcolor{header}\textcolor{white}{P2}} &
  \textbf{\cellcolor{header}\textcolor{white}{P3}} &
  \textbf{\cellcolor{header}\textcolor{white}{P4}} &
  \textbf{\cellcolor{header}\textcolor{white}{P5}} &
  \textbf{\cellcolor{header}\textcolor{white}{P6}} &
  \textbf{\cellcolor{header}\textcolor{white}{P7}}
  \bigstrut\\
\hline
BKP &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\hline
\multirow{4}[8]{*}{BKP-PC} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\hline
\multicolumn{1}{|l|}{\multirow{2}[4]{*}{Increase/Decrease\_Value\_Of}} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\cline{2-9}\multicolumn{1}{|l|}{} &
   &
   &
   &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{} &
  
  \bigstrut\\
\hline
\end{tabular}%

==> table_lr3.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\LARGE
%\rowcolors{1}{}{lightmyblue}
\resizebox {1\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'Sheet2'
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
		\toprule[1.5 pt]
		\textbf{\cellcolor{header}\textcolor{white}{Employed Model}} &
		\textbf{\cellcolor{header}\textcolor{white}{Works}} &
		\textbf{\cellcolor{header}\textcolor{white}{P1}} &
		\textbf{\cellcolor{header}\textcolor{white}{P2}} &
		\textbf{\cellcolor{header}\textcolor{white}{P3}} &
		\textbf{\cellcolor{header}\textcolor{white}{P4}} &
		\textbf{\cellcolor{header}\textcolor{white}{P5}} &
		\textbf{\cellcolor{header}\textcolor{white}{P6}} &
		\textbf{\cellcolor{header}\textcolor{white}{P7}} 
		%\textbf{\cellcolor{header}\textcolor{white}{P8}} 

		\bigstrut\\
		\hline
		BKP &
		\begin{tabular}[t]{@{}c@{}} \cite{karlsson_optimizing_1997,jung_optimizing_1998,zhang_multi_objective_2007,baker_search_2006,finkelstein2009search,zhang2011comparing,del2010ant,kumari2012software} \phantom{sssssssssssss} \end{tabular} &
		NO &
		NO &
		NO &
		NO &
		NO &
		NO &
		NO
		\bigstrut\\
		\hline
		\multirow{4}[9]{*}{BKP-PC} &
		\begin{tabular}[t]{@{}c@{}} \cite{veerapen2015integer,brasil_multiobjective_2012,sagrado_multi_objective_2013,bagnall_next_2001,greer_software_2004,boschetti_lagrangian_2014,ruhe_quantitative_2003,van2011quantitative,zhang2010search,tonella2010using,freitas2011software}\\ \cite{colares_new_2009,saliu2007bi,saliu2005supporting,jiang2010hybrid,van2005determination,ngo2009optimized,chen2013ant,del2011requirements,araujo2016architecture,colares2009new,pitangueira2016risk}\end{tabular} &
		NO  &
		NO  &
		NO  &
		NO  &
		YES &
		NO  &
		NO  
		\bigstrut\\
		%\cdashline{2-9}
		\cline{2-10} &
		\cite{van2008software,ngo_wicked_2008} &
		YES &
		YES &
		YES &
		NO  &
		YES &
		NO  &
		NO   
		\bigstrut\\
		\cline{2-10} &
		\cite{tonella2013interactive,xuan2012solving,saliu2005software} &
		YES &
		NO  &
		NO  &
		NO  &
		YES &
		NO  &
		NO 
		\bigstrut\\
		\hline
		\multicolumn{1}{|l|}{\multirow{2}[4]{*}{Increase-Decrease}} &
		\cite{li_integrated_2010,sagrado_multi_objective_2013,Zhang_RIM_2013} (subsets of size 2) &
		YES &
		NO  &
		YES &
		NO  &
		YES &
		NO  &
		YES 
		\bigstrut\\
		\cline{2-10}\multicolumn{1}{|l|}{} &
		\cite{van_den_akker_flexible_2005} (subsets of any size) &
		YES &
		YES &
		NO  &
		NO  &
		YES &
		NO  &
		YES 
		\bigstrut\\
		\hline
	\end{tabular}%
}


==> table_lr4.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\LARGE
%\rowcolors{1}{}{lightmyblue}
\resizebox {1\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'Sheet2'
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
		\toprule[1.5 pt]
		\textbf{\cellcolor{header}\textcolor{white}{Technique}} &
		\textbf{\cellcolor{header}\textcolor{white}{Employed by}} &
		\textbf{\cellcolor{header}\textcolor{white}{P1}} &
		\textbf{\cellcolor{header}\textcolor{white}{P2}} &
		\textbf{\cellcolor{header}\textcolor{white}{P3}} &
		\textbf{\cellcolor{header}\textcolor{white}{P4}} &
		\textbf{\cellcolor{header}\textcolor{white}{P5}} &
		\textbf{\cellcolor{header}\textcolor{white}{P6}} &
		\textbf{\cellcolor{header}\textcolor{white}{P7}} 
		%\textbf{\cellcolor{header}\textcolor{white}{P8}} 

		\bigstrut\\
		\hline
		BK &
		\begin{tabular}[t]{@{}c@{}} \cite{karlsson_optimizing_1997,jung_optimizing_1998,zhang_multi_objective_2007,baker_search_2006,finkelstein2009search,zhang2011comparing,del2010ant,kumari2012software} \phantom{sssssssssssss} \end{tabular} &
		NO &
		NO &
		NO &
		NO &
		NO &
		NO &
		NO
		\bigstrut\\
		\hline
		\multirow{4}[9]{*}{PCBK} &
		\begin{tabular}[t]{@{}l@{}} \cite{veerapen2015integer,brasil_multiobjective_2012,sagrado_multi_objective_2013,bagnall_next_2001,greer_software_2004,boschetti_lagrangian_2014,ruhe_quantitative_2003,van2011quantitative,zhang2010search,tonella2010using,freitas2011software}\\ \cite{colares_new_2009,saliu2007bi,saliu2005supporting,jiang2010hybrid,van2005determination,ngo2009optimized,chen2013ant,del2011requirements,araujo2016architecture,colares2009new,pitangueira2016risk}\\\cite{van2008software,ngo_wicked_2008,tonella2013interactive,xuan2012solving,saliu2005software}\end{tabular} &
		NO  &
		NO  &
		NO  &
		NO  &
		NO  &
		YES  &
		NO  
		\bigstrut\\
		\hline
		\multicolumn{1}{|l|}{\multirow{2}[4]{*}{Increase-Decrease}} &
		\cite{li_integrated_2010,sagrado_multi_objective_2013,Zhang_RIM_2013} (subsets of size 2) &
		YES &
		NO  &
		YES &
		NO  &
		NO  &
		YES &
		YES 
		\bigstrut\\
		\cline{2-10}\multicolumn{1}{|l|}{} &
		\cite{van_den_akker_flexible_2005} (subsets of any size) &
		YES &
		YES &
		NO  &
		NO  &
		NO  &
		YES &
		YES 
		\bigstrut\\
		\hline
		SBK &
		\begin{tabular}[t]{@{}c@{}} \cite{pitangueira2017minimizing,li2016value,li2014robust} \phantom{sssssssssssss} \end{tabular} &
		NO &
		NO &
		NO &
		NO &
		NO &
		NO &
		YES
		\bigstrut\\
		\hline
	\end{tabular}%
}


==> table_lr_new.tex <==
	\begin{tabular}{lllllll}
		&                                                                                         &                                                                                                               &                                                                                                                                                                                                                                                                         &                                                                                                     &                                                               &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Categories}}                                                & \multicolumn{1}{l|}{\textbf{BKP Models}}                                                                      & \multicolumn{1}{l|}{\textbf{BKP-PC Models}}                                                                                                                                                                                                                             & \multicolumn{2}{l|}{\textbf{Increase/Decrease-Value-of Models}}                                                                                                     &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Works from the Literature}                                          & \multicolumn{1}{l|}{\cite\{karlsson\_optimizing\_1997,jung\_optimizing\_1998,zhang\_multi\_objective\_2007\}} & \multicolumn{1}{l|}{\cite\{brasil\_multiobjective\_2012,li\_integrated\_2010,sagrado\_multi\_objective\_2013,boschetti\_lagrangian\_2014,brasil\_multiobjective\_2012,brasil\_multiobjective\_2012,bagnall\_next\_2001,Greer\_evolutionary\_2004,baker\_search\_2006\}} & \multicolumn{1}{l|}{\cite\{li\_integrated\_2010,sagrado\_multi\_objective\_2013,Zhang\_RIM\_2013\}} & \multicolumn{1}{l|}{\cite\{van\_den\_akker\_flexible\_2005\}} &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}considers explicit value dependencies}      & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}NO}                                                               & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}YES}                                                                                                                                                                                                                        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}YES}                                                    & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}YES}              &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{considers implicit value dependencies}                              & \multicolumn{1}{l|}{NO}                                                                                       & \multicolumn{1}{l|}{YES}                                                                                                                                                                                                                                                & \multicolumn{1}{l|}{NO}                                                                             & \multicolumn{1}{l|}{NO}                                       &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{considers qualities (positivity/negativity) of  value dependencies} & \multicolumn{1}{l|}{NO}                                                                                       & \multicolumn{1}{l|}{YES}                                                                                                                                                                                                                                                & \multicolumn{1}{l|}{YES}                                                                            & \multicolumn{1}{l|}{NO}                                       &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{considers strengths of value dependencies}                          & \multicolumn{1}{l|}{NO}                                                                                       & \multicolumn{1}{l|}{NO}                                                                                                                                                                                                                                                 & \multicolumn{1}{l|}{NO}                                                                             & \multicolumn{1}{l|}{NO}                                       &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{considers simultaneous positive and negative value dependencies}    & \multicolumn{1}{l|}{NO}                                                                                       & \multicolumn{1}{l|}{YES}                                                                                                                                                                                                                                                & \multicolumn{1}{l|}{NO}                                                                             & \multicolumn{1}{l|}{NO}                                       &  \\ \cline{2-6}
		\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{is prone to SDP}                                                    & \multicolumn{1}{l|}{NO}                                                                                       & \multicolumn{1}{l|}{YES}                                                                                                                                                                                                                                                & \multicolumn{1}{l|}{NO}                                                                             & \multicolumn{1}{l|}{NO}                                       &  \\ \cline{2-6}
		&                                                                                         &                                                                                                               &                                                                                                                                                                                                                                                                         &                                                                                                     &                                                               &  \\
		&                                                                                         &                                                                                                               &                                                                                                                                                                                                                                                                         &                                                                                                     &                                                               &  \\
		&                                                                                         &                                                                                                               &                                                                                                                                                                                                                                                                         &                                                                                                     &                                                               &  \\
		&                                                                                         &                                                                                                               &                                                                                                                                                                                                                                                                         &                                                                                                     &                                                               &  \\
		&                                                                                         &                                                                                                               &                                                                                                                                                                                                                                                                         &                                                                                                     &                                                               &  \\
		&                                                                                         &                                                                                                               &                                                                                                                                                                                                                                                                         &                                                                                                     &                                                               & 
	\end{tabular}


==> table_lr_old.tex <==
\rowcolors{1}{}{lightgray}
\LARGE\resizebox {1\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'Sheet1'
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{l|l|l|l|l}
	\hline
	\multicolumn{1}{l|}{\multirow{2}[4]{*}{\textbf{Selection Model}}} &
	\multicolumn{1}{l|}{\multirow{2}[4]{*}{\textbf{BKP}}} &
	\multicolumn{1}{l|}{\multirow{2}[4]{*}{\textbf{BKP-PC}}} &
	\multicolumn{2}{c}{\textbf{Increase/Decrease-Value-of}}
	\bigstrut\\
	\cline{4-5}\multicolumn{1}{c|}{} &
	\multicolumn{1}{l|}{} &
	\multicolumn{1}{l|}{} &
	\multicolumn{1}{l|}{Subsets of Size 2 Only} &
	\multicolumn{1}{l}{Subsets of Any Size}
	\bigstrut\\
	\hline
	\multicolumn{1}{l|}{Sample works from the  literature} &
	\cite{karlsson_optimizing_1997,jung_optimizing_1998,zhang_multi_objective_2007}  &
	\cite{brasil_multiobjective_2012,li_integrated_2010,sagrado_multi_objective_2013,Greer_evolutionary_2004,boschetti_lagrangian_2014,bagnall_next_2001,baker_search_2006} &
	\cite{li_integrated_2010,sagrado_multi_objective_2013,Zhang_RIM_2013} &
	\cite{van_den_akker_flexible_2005}
	\bigstrut\\
	\hline
	Considers explicit value dependencies &
	NO &
	YES &
	YES &
	YES
	\bigstrut[t]\\
	Considers implicit value dependencies &
	NO &
	YES &
	NO &
	NO
	\\
	Considers qualities (positivity/negativity) of  value dependencies &
	NO &
	YES &
	YES &
	NO
	\\
	Considers strengths of value dependencies &
	NO &
	NO &
	NO &
	NO
	\\
	Considers simultaneous positive and negative value dependencies  &
	NO &
	YES &
	NO &
	NO
	\\
	Is prone to SDP &
	NO &
	YES &
	NO &
	NO
	\bigstrut[b]\\
	\hline
\end{tabular}
}




==> table_precede.tex <==
\huge\resizebox {1\textwidth }{!}{
\begin{tabular}{lllllllllllllllllllllllllllll}
\toprule[1.5pt]
\textbf{\cellcolor{black}\textcolor{white}{}}& \textbf{\cellcolor{black}\textcolor{white}{$f_{1}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{2}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{3}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{4}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{5}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{6}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{7}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{8}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{9}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{10}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{11}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{12}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{13}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{14}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{15}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{16}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{17}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{18}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{19}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{20}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{21}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{22}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{23}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{24}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{25}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{26}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{27}$}}
\\\midrule \addlinespace[0.4ex]
\textbf{\cellcolor{black}\textcolor{white}{$f_{1}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{2}$}}& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{3}$}}& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{4}$}}& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{5}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{6}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{7}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{8}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{9}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{10}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{11}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{12}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{13}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{14}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{15}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{16}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{17}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{18}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{19}$}}& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{20}$}}& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{21}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{22}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{23}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{24}$}}& \cellcolor{gray!30}$+1.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{25}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{26}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& \cellcolor{gray!30}$+1.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{27}$}}& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$& $\pm0.00$\\
\addlinespace[0.4ex]\toprule[1.5pt]
\end{tabular}}

==> table_rho.tex <==
\huge\resizebox {1\textwidth }{!}{
\begin{tabular}{lllllllllllllllllllllllllllll}
\toprule[1.5pt]
\textbf{\cellcolor{black}\textcolor{white}{}}& \textbf{\cellcolor{black}\textcolor{white}{$f_{1}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{2}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{3}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{4}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{5}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{6}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{7}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{8}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{9}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{10}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{11}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{12}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{13}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{14}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{15}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{16}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{17}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{18}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{19}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{20}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{21}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{22}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{23}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{24}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{25}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{26}$}}
& \textbf{\cellcolor{black}\textcolor{white}{$f_{27}$}}
\\\midrule \addlinespace[0.4ex]
\textbf{\cellcolor{black}\textcolor{white}{$f_{1}$}}& $\pm0.00$& $+0.14$& $+0.09$& $+0.03$& $+0.14$& $+0.01$& $+0.01$& $+0.16$& $+0.03$& $+0.03$& $-0.02$& $+0.11$& $+0.03$& $+0.11$& $+0.15$& $+0.09$& $+0.01$& $-0.04$& $-0.04$& $-0.04$& $-0.02$& $+0.06$& $+0.14$& $+0.14$& $-0.14$& $-0.18$& $-0.01$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{2}$}}& $+0.16$& $\pm0.00$& $+0.20$& $+0.47$& $+1.00$& $+0.07$& $+0.02$& $+0.25$& $+0.47$& $+0.47$& $+0.25$& $+0.07$& $+0.47$& $+0.22$& $+0.24$& $+0.43$& $+0.22$& $+0.24$& $+0.12$& $+0.17$& $+0.18$& $+0.19$& $+1.00$& $+1.00$& $+0.18$& $+0.00$& $+0.15$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{3}$}}& $+0.18$& $+0.37$& $\pm0.00$& $+0.40$& $+0.37$& $-0.00$& $+0.15$& $+0.47$& $+0.40$& $+0.40$& $+0.33$& $-0.15$& $+0.40$& $+0.68$& $+0.50$& $+0.35$& $-0.07$& $+0.07$& $+0.01$& $+0.09$& $+0.48$& $+0.33$& $+0.37$& $+0.37$& $+0.00$& $-0.06$& $+0.02$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{4}$}}& $+0.05$& $+0.72$& $+0.32$& $\pm0.00$& $+0.72$& $+0.30$& $-0.02$& $+0.42$& $+1.00$& $+1.00$& $+0.39$& $+0.03$& $+1.00$& $+0.33$& $+0.39$& $+0.40$& $+0.12$& $+0.37$& $-0.00$& $+0.25$& $+0.27$& $+0.30$& $+0.72$& $+0.72$& $+0.27$& $-0.11$& $+0.24$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{5}$}}& $+0.16$& $+1.00$& $+0.20$& $+0.47$& $\pm0.00$& $+0.07$& $+0.02$& $+0.25$& $+0.47$& $+0.47$& $+0.25$& $+0.07$& $+0.47$& $+0.22$& $+0.24$& $+0.43$& $+0.22$& $+0.24$& $+0.12$& $+0.17$& $+0.18$& $+0.19$& $+1.00$& $+1.00$& $+0.18$& $+0.00$& $+0.15$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{6}$}}& $+0.02$& $+0.11$& $-0.00$& $+0.33$& $+0.11$& $\pm0.00$& $-0.05$& $+0.13$& $+0.33$& $+0.33$& $+0.14$& $+0.32$& $+0.33$& $+0.05$& $+0.09$& $-0.03$& $-0.19$& $+0.08$& $-0.37$& $+0.27$& $-0.25$& $-0.03$& $+0.11$& $+0.11$& $+0.04$& $-0.49$& $+0.30$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{7}$}}& $+0.01$& $+0.04$& $+0.11$& $-0.02$& $+0.04$& $-0.04$& $\pm0.00$& $-0.11$& $-0.02$& $-0.02$& $+0.21$& $-0.14$& $-0.02$& $+0.12$& $-0.14$& $-0.04$& $-0.10$& $-0.16$& $-0.09$& $+0.17$& $-0.03$& $-0.23$& $+0.04$& $+0.04$& $-0.04$& $+0.02$& $+0.16$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{8}$}}& $+0.33$& $+0.46$& $+0.47$& $+0.51$& $+0.46$& $+0.14$& $-0.15$& $\pm0.00$& $+0.51$& $+0.51$& $+0.24$& $-0.07$& $+0.51$& $+0.54$& $+0.70$& $+0.25$& $+0.01$& $+0.21$& $-0.11$& $-0.09$& $+0.36$& $+0.43$& $+0.46$& $+0.46$& $-0.05$& $-0.24$& $-0.00$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{9}$}}& $+0.05$& $+0.72$& $+0.32$& $+1.00$& $+0.72$& $+0.30$& $-0.02$& $+0.42$& $\pm0.00$& $+1.00$& $+0.39$& $+0.03$& $+1.00$& $+0.33$& $+0.39$& $+0.40$& $+0.12$& $+0.37$& $-0.00$& $+0.25$& $+0.27$& $+0.30$& $+0.72$& $+0.72$& $+0.27$& $-0.11$& $+0.24$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{10}$}}& $+0.05$& $+0.72$& $+0.32$& $+1.00$& $+0.72$& $+0.30$& $-0.02$& $+0.42$& $+1.00$& $\pm0.00$& $+0.39$& $+0.03$& $+1.00$& $+0.33$& $+0.39$& $+0.40$& $+0.12$& $+0.37$& $-0.00$& $+0.25$& $+0.27$& $+0.30$& $+0.72$& $+0.72$& $+0.27$& $-0.11$& $+0.24$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{11}$}}& $-0.04$& $+0.49$& $+0.34$& $+0.49$& $+0.49$& $+0.16$& $+0.29$& $+0.25$& $+0.49$& $+0.49$& $\pm0.00$& $-0.04$& $+0.49$& $+0.42$& $+0.20$& $+0.26$& $+0.10$& $+0.28$& $+0.00$& $+0.42$& $+0.36$& $-0.02$& $+0.49$& $+0.49$& $+0.24$& $-0.06$& $+0.24$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{12}$}}& $+0.15$& $+0.08$& $-0.10$& $+0.03$& $+0.08$& $+0.22$& $-0.11$& $-0.04$& $+0.03$& $+0.03$& $-0.02$& $\pm0.00$& $+0.03$& $-0.10$& $-0.06$& $+0.02$& $-0.02$& $-0.06$& $-0.04$& $+0.17$& $-0.26$& $-0.11$& $+0.08$& $+0.08$& $+0.01$& $-0.20$& $+0.17$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{13}$}}& $+0.05$& $+0.72$& $+0.32$& $+1.00$& $+0.72$& $+0.30$& $-0.02$& $+0.42$& $+1.00$& $+1.00$& $+0.39$& $+0.03$& $\pm0.00$& $+0.33$& $+0.39$& $+0.40$& $+0.12$& $+0.37$& $-0.00$& $+0.25$& $+0.27$& $+0.30$& $+0.72$& $+0.72$& $+0.27$& $-0.11$& $+0.24$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{14}$}}& $+0.25$& $+0.43$& $+0.71$& $+0.43$& $+0.43$& $+0.06$& $+0.17$& $+0.57$& $+0.43$& $+0.43$& $+0.42$& $-0.16$& $+0.43$& $\pm0.00$& $+0.59$& $+0.37$& $-0.00$& $+0.14$& $-0.11$& $+0.10$& $+0.46$& $+0.27$& $+0.43$& $+0.43$& $-0.06$& $-0.18$& $-0.03$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{15}$}}& $+0.32$& $+0.47$& $+0.52$& $+0.50$& $+0.47$& $+0.10$& $-0.20$& $+0.73$& $+0.50$& $+0.50$& $+0.20$& $-0.09$& $+0.50$& $+0.58$& $\pm0.00$& $+0.48$& $+0.10$& $+0.30$& $-0.01$& $-0.04$& $+0.42$& $+0.51$& $+0.47$& $+0.47$& $+0.02$& $-0.17$& $-0.13$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{16}$}}& $+0.14$& $+0.59$& $+0.25$& $+0.36$& $+0.59$& $-0.02$& $-0.04$& $+0.18$& $+0.36$& $+0.36$& $+0.18$& $+0.02$& $+0.36$& $+0.26$& $+0.33$& $\pm0.00$& $+0.31$& $+0.30$& $+0.25$& $+0.20$& $+0.25$& $+0.24$& $+0.59$& $+0.59$& $+0.23$& $+0.08$& $-0.01$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{17}$}}& $+0.02$& $+0.41$& $-0.07$& $+0.15$& $+0.41$& $-0.22$& $-0.13$& $+0.01$& $+0.15$& $+0.15$& $+0.10$& $-0.03$& $+0.15$& $-0.00$& $+0.10$& $+0.44$& $\pm0.00$& $+0.52$& $+0.49$& $+0.12$& $+0.33$& $+0.24$& $+0.41$& $+0.41$& $+0.42$& $+0.32$& $-0.01$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{18}$}}& $-0.10$& $+0.48$& $+0.08$& $+0.47$& $+0.48$& $+0.09$& $-0.23$& $+0.22$& $+0.47$& $+0.47$& $+0.28$& $-0.09$& $+0.47$& $+0.14$& $+0.30$& $+0.44$& $+0.54$& $\pm0.00$& $+0.29$& $+0.22$& $+0.46$& $+0.39$& $+0.48$& $+0.48$& $+0.57$& $+0.16$& $+0.07$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{19}$}}& $-0.08$& $+0.21$& $+0.01$& $-0.00$& $+0.21$& $-0.39$& $-0.11$& $-0.11$& $-0.00$& $-0.00$& $+0.00$& $-0.06$& $-0.00$& $-0.10$& $-0.01$& $+0.33$& $+0.47$& $+0.26$& $\pm0.00$& $+0.03$& $+0.31$& $+0.17$& $+0.21$& $+0.21$& $+0.35$& $+0.49$& $-0.11$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{20}$}}& $-0.07$& $+0.26$& $+0.08$& $+0.26$& $+0.26$& $+0.25$& $+0.19$& $-0.07$& $+0.26$& $+0.26$& $+0.33$& $+0.22$& $+0.26$& $+0.08$& $-0.03$& $+0.23$& $+0.10$& $+0.17$& $+0.03$& $\pm0.00$& $+0.01$& $-0.10$& $+0.26$& $+0.26$& $+0.36$& $-0.05$& $+0.42$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{21}$}}& $-0.03$& $+0.23$& $+0.33$& $+0.22$& $+0.23$& $-0.19$& $-0.03$& $+0.25$& $+0.22$& $+0.22$& $+0.24$& $-0.28$& $+0.22$& $+0.30$& $+0.28$& $+0.24$& $+0.23$& $+0.30$& $+0.22$& $+0.01$& $\pm0.00$& $+0.33$& $+0.23$& $+0.23$& $+0.23$& $+0.22$& $-0.09$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{22}$}}& $+0.12$& $+0.34$& $+0.32$& $+0.35$& $+0.34$& $-0.03$& $-0.29$& $+0.42$& $+0.35$& $+0.35$& $-0.01$& $-0.16$& $+0.35$& $+0.25$& $+0.48$& $+0.33$& $+0.23$& $+0.36$& $+0.17$& $-0.12$& $+0.47$& $\pm0.00$& $+0.34$& $+0.34$& $+0.24$& $+0.11$& $-0.01$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{23}$}}& $+0.16$& $+1.00$& $+0.20$& $+0.47$& $+1.00$& $+0.07$& $+0.02$& $+0.25$& $+0.47$& $+0.47$& $+0.25$& $+0.07$& $+0.47$& $+0.22$& $+0.24$& $+0.43$& $+0.22$& $+0.24$& $+0.12$& $+0.17$& $+0.18$& $+0.19$& $\pm0.00$& $+1.00$& $+0.18$& $+0.00$& $+0.15$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{24}$}}& $+0.16$& $+1.00$& $+0.20$& $+0.47$& $+1.00$& $+0.07$& $+0.02$& $+0.25$& $+0.47$& $+0.47$& $+0.25$& $+0.07$& $+0.47$& $+0.22$& $+0.24$& $+0.43$& $+0.22$& $+0.24$& $+0.12$& $+0.17$& $+0.18$& $+0.19$& $+1.00$& $\pm0.00$& $+0.18$& $+0.00$& $+0.15$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{25}$}}& $-0.25$& $+0.29$& $+0.00$& $+0.28$& $+0.29$& $+0.04$& $-0.04$& $-0.04$& $+0.28$& $+0.28$& $+0.20$& $+0.01$& $+0.28$& $-0.05$& $+0.02$& $+0.27$& $+0.36$& $+0.47$& $+0.32$& $+0.38$& $+0.29$& $+0.21$& $+0.29$& $+0.29$& $\pm0.00$& $+0.30$& $+0.27$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{26}$}}& $-0.37$& $+0.01$& $-0.06$& $-0.13$& $+0.01$& $-0.53$& $+0.02$& $-0.24$& $-0.13$& $-0.13$& $-0.06$& $-0.30$& $-0.13$& $-0.17$& $-0.16$& $+0.11$& $+0.31$& $+0.15$& $+0.50$& $-0.06$& $+0.31$& $+0.11$& $+0.01$& $+0.01$& $+0.34$& $\pm0.00$& $-0.11$\\
\textbf{\cellcolor{black}\textcolor{white}{$f_{27}$}}& $-0.01$& $+0.25$& $+0.01$& $+0.27$& $+0.25$& $+0.30$& $+0.19$& $-0.00$& $+0.27$& $+0.27$& $+0.20$& $+0.24$& $+0.27$& $-0.02$& $-0.11$& $-0.01$& $-0.01$& $+0.06$& $-0.10$& $+0.46$& $-0.12$& $-0.01$& $+0.25$& $+0.25$& $+0.28$& $-0.10$& $\pm0.00$\\
\addlinespace[0.4ex]\toprule[1.5pt]
\end{tabular}}

==> table_sigma.tex <==
\resizebox {0.5\textwidth }{!}{
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{lllll}
	\boldmath{}\textbf{$\sigma_{I,j}$}\unboldmath{} &
	\boldmath{}\textbf{$r_1$}\unboldmath{} &
	\boldmath{}\textbf{$r_2$}\unboldmath{} &
	\boldmath{}\textbf{$r_3$}\unboldmath{} &
	\boldmath{}\textbf{$r_4$}\unboldmath{}
	\\
	\boldmath{}\textbf{$r_1$}\unboldmath{} &
	&
	&
	&
	
	\\
	\boldmath{}\textbf{$r_2$}\unboldmath{} &
	&
	&
	&
	
	\\
	\boldmath{}\textbf{$r_3$}\unboldmath{} &
	&
	&
	&
	
	\\
	\boldmath{}\textbf{$r_4$}\unboldmath{} &
	&
	&
	&
	
	\\
\end{tabular}%
}


==> table_sim_design.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\resizebox {1\textwidth }{!}{
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{|l|l|l|l|l|}
	\cmidrule[1pt]{2-5}
	\multicolumn{1}{l|}{} 
	&
	\cellcolor{gray!30}\textbf{VDL=[0,1]} &
	\cellcolor{gray!30}\textbf{NVDL=[0,1]} &
	\cellcolor{gray!30}\textbf{PDL=[0,1]} & 
	\cellcolor{gray!30}\textbf{NPDL=[0,1]} 
	\bigstrut\\
	\hline
	\cellcolor{gray!30}$\%$\textbf{Budget=[0,100]} &
	NVDL=0.0,PDL=0.02,NPDL=0.0  &
	VDL=0.15,PDL=0.02,NPDL=0.0  &
	VDL=0.15,NVDL=0.0,NPDL=0.0 & 
	VDL=0.15,NVDL=0.0,PDL=0.02
	\bigstrut\\
	\hline
	\cellcolor{gray!30}\textbf{VDL=[0,1]} &
	&
	$\%$Budget=95, PDL=0.02, NPDL=0.0 &
	$\%$Budget=95,NVDL=0.0, NPDL=0.0 &
	$\%$Budget=95,NVDL=0.0, PDL=0.02
	\bigstrut\\
	\hline
	\cellcolor{gray!30}\textbf{NVDL=[0,1]} &
	&
	&
	$\%$Budget=95,VDL=0.15, NPDL=0.0 &
	$\%$Budget=95,VDL=0.15, PDL=0.02
	\bigstrut\\
	\hline
	\cellcolor{gray!30}\textbf{PDL=[0,1]} &
	&
	&
	& 
	$\%$Budget=95, VDL=0.15, NVDL=0.0 
	\bigstrut\\
	\bottomrule
\end{tabular}%
}

==> table_sim_design_all_previous.tex <==
% Table generated by Excel2LaTeX from sheet 'table_sim_design_all'
\resizebox {0.7\textwidth }{!}{
	\begin{tabular}{clllll}
	\toprule[1.5pt]
	\rowcolor{gray!30}
	\textbf{\cellcolor{black}\textcolor{white}{Simulation}} &
	\textbf{\cellcolor{black}\textcolor{white}{$\%$Budget}} &
	\textbf{\cellcolor{black}\textcolor{white}{VDL}} &
	\textbf{\cellcolor{black}\textcolor{white}{NVDL}} &
    \textbf{\cellcolor{black}\textcolor{white}{PDL}} &
	\textbf{\cellcolor{black}\textcolor{white}{NPDL}} 
	\bigstrut\\
	\rowcolor{gray!25}
	%\hline
	I &
	[0,1] &
	[0,1] &
	0.00&
	0.02 &
	0.00
	\bigstrut\\
	%\hline
	II &
	[0,1] &
	0.15 &
	[0,1] &
	0.02 &
	0.00
	\bigstrut\\
	\rowcolor{gray!25}
	%\hline
	III &
	[0,1] &
	0.15 &
	0.00&
	[0,1] &
	0.00
	\bigstrut\\
	%\hline
	IV &
	[0,1] &
	0.15 &
	0.00&
	0.02 &
	[0,1]
	\bigstrut\\
	\rowcolor{gray!25}
	%\hline
	V &
	0.95 &
	[0,1] &
	[0,1] &
	0.02 &
	0.00
	\bigstrut\\
	%\hline
	VI &
	0.95 &
	[0,1] &
	0.00&
	[0,1] &
	0.00
	\bigstrut\\
	\rowcolor{gray!25}
	%\hline
	VII &
	0.95 &
	[0,1] &
	0.00&
	0.02 &
	[0,1]
	\bigstrut\\
	%\hline
	VIII &
	0.95 &
	0.15 &
	[0,1] &
	[0,1] &
	0.00
	\bigstrut\\
	\rowcolor{gray!25}
	%\hline
	IX &
	0.95 &
	0.15 &
	[0,1] &
	0.02 &
	[0,1]
	\bigstrut\\
	\rowcolor{gray!25}
	%\hline
	X &
	0.95 &
	0.15 &
	0.00&
	[0,1] &
	[0,1]
	\bigstrut\\
	\bottomrule[1.5pt]
\end{tabular}
}


==> table_sim_scalability_design_previous.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\resizebox {0.75\textwidth }{!}{
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{lllllll}
	\toprule[1.5pt]
	\rowcolor{gray!30}
	\textbf{\cellcolor{black}\textcolor{white}{Simulation}} &
	\textbf{\cellcolor{black}\textcolor{white}{Size}} &
	\textbf{\cellcolor{black}\textcolor{white}{$\%$Budget}} &
	\textbf{\cellcolor{black}\textcolor{white}{VDL}} &
	\textbf{\cellcolor{black}\textcolor{white}{NVDL}} &
	\textbf{\cellcolor{black}\textcolor{white}{PDL}} &
	\textbf{\cellcolor{black}\textcolor{white}{NPDL}}
	\bigstrut\\
	\hline
	XI &
	[0,2000] &
	50 &
	0.15 &
	0.00 &
	0.02 &
	0.00
	\bigstrut\\ \rowcolor{gray!25}
	XII &
	200 &
	[0,100] &
	0.15 &
	0.00 &
	0.02 &
	0.00
    \bigstrut\\
	XIII &
	[0,1000] &
	[0,100] &
	0.15 &
	0.00 &
	0.02 &
	0.00
	\bigstrut\\	\rowcolor{gray!25}
	XIV &
	200 &
	50 &
	0.15 &
	0.00 &
	[0,0.007] &
	0.00
	\bigstrut\\	
	XV &
	200 &
	50 &
	0.15 &
	0 &
    [0.007,1] &
	0.00
	\bigstrut\\ \rowcolor{gray!25}
	XVI &
	200 &
	50 &
	[0,1] &
	[0,1] &
	0.02 &
	0.00
	\bigstrut\\
	XVII &
	200 &
	50 &
	0.15 &
	0.00 &
	[0,1] &
	0.00
	\bigstrut\\ \rowcolor{gray!25}
	XVIII &
	200 &
	50 &
	0.15 &
	0.00 &
	0.02 &
	[0,1]
	\bigstrut\\
	XIX &
	200 &
	50 &
	0.15 &
	0.00 &
	[0,1] &
	[0,1]
	\bigstrut\\ 
	\bottomrule[1.5pt]
\end{tabular}
}

==> table_types_intrinsic.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\LARGE
%\rowcolors{1}{}{myblue!20}
\resizebox {1\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'Sheet1'
	\begin{tabular}{|l|l|l|}
		\toprule[1.5 pt]
		\textbf{\cellcolor{header}\textcolor{white}{Dependency Type}} &
		\textbf{\cellcolor{header}\textcolor{white}{Description}} &
		\textbf{\cellcolor{header}\textcolor{white}{Example}}
		\bigstrut\\
		\hline
		\begin{tabular}[c]{@{}l@{}}Constrain~\cite{zhang_investigating_2014,k_process_centered_1996}\end{tabular} &
	    \begin{tabular}[c]{@{}l@{}}\textit{ }\textbullet\textit{ }One requirement is a constraint of another requirement.\end{tabular}  &
		\begin{tabular}[c]{@{}l@{}}			
			\textit{ }\textbullet\textit{ } $r_1:$ system should respond to users in 3 seconds \\
			\textit{ }\textbullet\textit{ } $r_2:$ users search books using book title or ID \\
			\textit{ }\textbullet\textit{ } $r_1$ constrains $r_2$
		\end{tabular}
		\bigstrut\\ \hline
		
		\begin{tabular}[c]{@{}l@{}}Precede~\cite{zhang_investigating_2014}, Precondition~\cite{k_process_centered_1996}, Requires~\cite{dahlstedt2005requirements}\end{tabular} &
		\begin{tabular}[c]{@{}l@{}}\textit{ }\textbullet\textit{ } If function A precedes function B\end{tabular} &
		\begin{tabular}[c]{@{}l@{}}			
			\textit{ }\textbullet\textit{ } $r_1:$ a client initiates a valuation request and the system checks the quality of the request\\
			\textit{ }\textbullet\textit{ } $r_2:$ users search books using book title or ID\\
			\textit{ }\textbullet\textit{ } $r_1$ precedes $r_2$\\
		\end{tabular}
		\bigstrut\\ \hline
		
		\begin{tabular}[c]{@{}l@{}}Be\_similar\_to~\cite{zhang_investigating_2014}, Similar~\cite{k_process_centered_1996}, Similar\_to~\cite{dahlstedt2005requirements}\end{tabular} &
		\begin{tabular}[c]{@{}l@{}}
				\textit{ }\textbullet\textit{ } (a) If two requirements share similar data information.\\ 
				\textit{ }\textbullet\textit{ } (b) If two requirements complete similar tasks.
		\end{tabular} &
		\begin{tabular}[c]{@{}l@{}}
				\textit{ }\textbullet\textit{ } (a) Adding a new book record is similar to modifying an old book as they share the book record.\\
				\textit{ }\textbullet\textit{ } (b) A property valuation could be complemented through curbside or desktop valuation.
		\end{tabular}
		\bigstrut\\ \hline
		
		\begin{tabular}[c]{@{}l@{}}Conflicts~\cite{zhang_investigating_2014,k_process_centered_1996}, Conflicts\_with~\cite{dahlstedt2005requirements}\end{tabular} &
		\begin{tabular}[c]{@{}l@{}} \textit{ }\textbullet\textit{ }One requirement may negatively impact another one.\end{tabular} &
		\textit{ }\textbullet\textit{ } Security may conflicts with performance.
		\bigstrut\\ \hline
		
		\begin{tabular}[c]{@{}l@{}}Be\_exception\_of~\cite{zhang_investigating_2014}\end{tabular} &
		\begin{tabular}[c]{@{}l@{}}\textit{ }\textbullet\textit{ }One requirement is an exceptional event of another one.\end{tabular} &
		\begin{tabular}[c]{@{}l@{}}
			\textit{ }\textbullet\textit{ } $r_1:$ A user inputs a null username and  system  reminds  him to correct it.\\
			\textit{ }\textbullet\textit{ } $r_2:$ A  user inputs his  username and  password  and  system checks validity of his information.\\
			\textit{ }\textbullet\textit{ } $r_1$ is an exception of $r_2$. 
		\end{tabular}
		\bigstrut\\ \hline
		
		\begin{tabular}[c]{@{}l@{}}Evolve\_into~\cite{zhang_investigating_2014}, Replaces~\cite{k_process_centered_1996}, Satisfies~\cite{k_process_centered_1996},\\ Based\_on~\cite{k_process_centered_1996}, Changes\_to~\cite{dahlstedt2005requirements}\end{tabular} &
		\begin{tabular}[c]{@{}l@{}} \textbullet\textit{ } Requirement $r_1$ is a new version of $r_2$. \end{tabular} &
		\begin{tabular}[c]{@{}l@{}}
			\textit{ }\textbullet\textit{ } $r_1:$ clients  use a desktop  PC  to upload  reports.\\
			\textit{ }\textbullet\textit{ } $r_2:$ clients use PDA to upload reports.\\
			\textit{ }\textbullet\textit{ } $r_1$ evolves into $r_2$. \\
		\end{tabular}
		\bigstrut\\ \hline
		
		\begin{tabular}[c]{@{}l@{}}Refines~\cite{zhang_investigating_2014,k_process_centered_1996}, Refines\_to~\cite{dahlstedt2005requirements}\end{tabular}&
		\begin{tabular}[c]{@{}l@{}} \textbullet\textit{ }One requirement is refined by more specific requirements.\end{tabular} &
		\begin{tabular}[c]{@{}l@{}}
			\textit{ }\textbullet\textit{ } $r_1:$ a valuer submit a valuation report.\\
			\textit{ }\textbullet\textit{ } $r_2:$ a valuer submits a report through web system.\\
			\textit{ }\textbullet\textit{ } $r_1$ is refined as $r_2$. 
		\end{tabular}
		\bigstrut\\
		\bottomrule[1.5pt]
	\end{tabular}
	}%


==> table_types_others.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
    \resizebox {1\textwidth }{!}{\begin{tabular}{|<{\centering}m{5cm}|<{\centering}m{10cm}|<{\centering}m{10cm}|<{\centering}m{5cm}|<{\centering}m{5cm}|}
\Xhline{4\arrayrulewidth}
\textbf{Dependency type} &
\textbf{Description} &
\textbf{Example} &
\textbf{Has Value (Dollars or Customer Satisfaction) Influences? }&
\textbf{Has Cost Influences?}
\bigstrut\\
\hline
Refined\_to 
& A higher-level requirement is refined by a number of more specific
requirements. 
& For a website, the requirement $r_1:$ \textit{authenticate users} can be refined to a more specific requirement $r_2:$ \textit{check user-name and password of users}.  
& YES~\cite{Robinson_RIM_2003,axel_reasoning_2004}. 
& YES~\cite{zhang_investigating_2014}

\bigstrut\\
\hline
Requires 
& Satisfaction of requirement $r_1$ to some extent \cite{dahlstedt_requirements_2005} depends on the satisfaction of requirement $r_2$. In case the dependency is strong $r_1$ can not be satisfied to any extent without $r_2$ in other cases, $r_1$ can still be partially satisfied without $r_2$ 
& Examples 1(Strong dependency): Sending an email requires a network connection, but not the opposite~\cite{carlshamre_industrial_2001} Examples 2(Week dependency):   
& YES~\cite{carlshamre_industrial_2001,carlshamre_release_2002,zhang_investigating_2014,dahlstedt_moulding_2003,dahlstedt_requirements_2005}. 
& YES~\cite{zhang_investigating_2014}

\bigstrut\\
\hline
Conflicts\_with
& Satisfaction of requirement $r_1$ strongly depends on the dissatisfaction of requirement $r_2$ to the extent that $r_1$ can not be satisfied to any extent when $r_2$ is even partially satisfied 
& If one requirement states that “All personnel should be able to search for information about both products and customers” and another states that “Only personnel with security status A should be able to search for customers classified as military related,” these two contradict each other, and cannot be simultaneously satisfied~\cite{dahlstedt_requirements_2005}.&
YES~\cite{carlshamre_industrial_2001,carlshamre_release_2002,zhang_investigating_2014,dahlstedt_moulding_2003,dahlstedt_requirements_2005}.
& YES~\cite{zhang_investigating_2014}

\bigstrut\\
\hline
AND 
& Is a bidirectional form of \texit{Requires} relation in which none of the AND-ed relations can be satisfied without the other one being fully satisfied. 
& a printer requires a driver to function, and the driver requires a printer to function~\cite{carlshamre_industrial_2001}. 
& YES, and discussed in the literature~\cite{carlshamre_industrial_2001,carlshamre_release_2002,zhang_investigating_2014,dahlstedt_moulding_2003,dahlstedt_requirements_2005}
& YES~\cite{zhang_investigating_2014}

\bigstrut\\
\hline
Increase/Decrease Value of 
& A requirement increases/decreases the value of another requirement without influencing its satisfaction. 
& Example 1: A detailed online manual may decrease the customer value of a printed manual~\cite{carlshamre_industrial_2001}. Example 2: The customer satisfaction of including a planning calendar into a mobile phone will probably increase if it is possible to synchronize this with planning calendars used on PCs 
& YES, and discussed in the literature~\cite{carlshamre_industrial_2001,carlshamre_release_2002,zhang_investigating_2014,dahlstedt_moulding_2003,dahlstedt_requirements_2005}.
& UNSPECIFIED

\bigstrut\\
\hline
Increase/Decrease Cost of 
& A requirement increases/decreases the cost of another requirement without influencing its satisfaction. 
& A requirement stating that ‘no response time should be longer than 1 second’ will typically increase the cost of implementing many other requirements~\cite{carlshamre_industrial_2001}. 
& NO 
& YES, and discussed in the literature~\cite{carlshamre_industrial_2001,carlshamre_release_2002,zhang_investigating_2014,dahlstedt_moulding_2003,dahlstedt_requirements_2005}.

\bigstrut\\
\Xhline{4\arrayrulewidth}
\end{tabular}}

==> table_types_robinson.tex <==
\resizebox {1\textwidth }{!}{\begin{tabular}{|l|l|}
\Xhline{4\arrayrulewidth}
\textbf{Dependency type} &
\textbf{Description} 

\bigstrut\\
\hline
Positive Influence(Interaction) 
& Increasing the satisfaction(value) of requirement $r_1$ will increase the satisfaction(value) of requirement $r_2$.

\bigstrut\\
\hline
Negative Influence(Interaction) 
& Increasing the satisfaction(value) of requirement $r_1$ will decreases the satisfaction(value) of requirement $r_2$. 

\bigstrut\\
\hline
Unspecified Influence(Interaction)
& Changing the satisfaction(value) of requirement $r_1$ has an unspecified influence on satisfaction(value) of requirement $r_2$.

\bigstrut\\
\hline
No Influence (Interaction) 
& Changing the satisfaction(value) of requirement $r_1$ has no influence on satisfaction(value) of requirement $r_2$. 

\bigstrut\\
\Xhline{4\arrayrulewidth}
\end{tabular}}

==> table_types_zhang.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\large\resizebox {1\textwidth }{!}{\begin{tabular}{|<{\centering}m{1.95cm}|<{\centering}m{4.8cm}|<{\centering}m{5.2cm}|<{\centering}m{8cm}|<{\centering}m{12cm}|}
\Xhline{4\arrayrulewidth}
\textbf{Category} &
\textbf{Types in Zhanng's model} &
\textbf{Corresponding types in other models} &
\textbf{Definition} &
\textbf{Example}

%--------------------------------------------------------
\bigstrut\\
\Xhline{4\arrayrulewidth}
intrinsic
& Constrain
& Constrain~\cite{k_process_centered_1996} 
& One requirement is a constraint of another requirement. This kind of dependency can represent crosscutting relationships among requirements.
& ‘system should respond to users in 3 seconds, constrains ‘book search function’ (user searches books using book title or ID).
%--------------------------------------------------------
\bigstrut\\
\cline{2-5} 
& Precede
& Precondition~\cite{k_process_centered_1996}, Requires~\cite{dahlstedt_requirements_2005}
& If function A precedes function B, A is a precondition of B.
& Given Requirement A:‘a client proposes the valuation request and system checks the quality of request’ and Requirement B:‘after the quality of request is checked, system allocates the valuation task to a valuer’, then A precedes B.
%--------------------------------------------------------
\bigstrut\\
\cline{2-5} 
& Be\_similar\_to
& Similar~\cite{k_process_centered_1996}, Similar\_to~\cite{dahlstedt_requirements_2005}
& a) If two requirements share similar data information, they are similar to each other. b) If two requirements complete similar tasks, they are similar to each other.
& a) Requirement ‘system administrator adds a new book re-cord’ is similar to ‘system administrator modiﬁes an old book record’. Book record in these two requirements is identical. b) After a client proposes a property valuation request, one valuer can choose from several options to evaluate the property,such as ‘desktop valuation’, ‘curbside valuation’or‘full evaluation’ Then these options (requirements) are similar to each other.
%--------------------------------------------------------
\bigstrut\\
\cline{2-5} 
& Conflict
& Conflicts~\cite{k_process_centered_1996}, Conflicts\_with~\cite{dahlstedt_requirements_2005}
& Implementation of one requirement negatively impacts another requirement.  
& Increasing security might negatively impact system performance.
%--------------------------------------------------------
\bigstrut\\
\cline{2-5} 
& Be\_exception\_of
& New dependency type
& One requirement describes an exceptional event of another requirement.
&‘‘A user inputs a null username and system reminds him to input his correct username’’ is an exceptional event of ‘‘a user inputs his username and password and system checks validity of his information’’.
%--------------------------------------------------------
\bigstrut\\
\cline{2-5} 
&Evolve\_into
& Replaces~\cite{k_process_centered_1996}, Satisfies~\cite{k_process_centered_1996}, Based\_on~\cite{k_process_centered_1996}, Changes\_to~\cite{dahlstedt_requirements_2005}
&If requirement B is a new version of requirement A, then A evolves into B. This type of dependency is used
to trace and compare different versions of requirement documents.
&‘‘Clients use a desktop PC to upload reports’’ evolves into ‘‘clients use PDA to upload reports’’.
%--------------------------------------------------------
\bigstrut\\
\cline{2-5} 
& Refine
& Refines~\cite{k_process_centered_1996}, Refines\_to~\cite{dahlstedt_requirements_2005}
& One requirement is refined by more specific requirements. 
&‘A valuer submit a valuation report’ is reﬁned as ‘a valuer submits a report through web system’,‘a valuer submits a report through PDA’.
%--------------------------------------------------------
\bigstrut\\
\hline
Additional
&Increase/Decrease\_cost\_of 
& Increase/Decrease\_cost\_of~\cite{dahlstedt_requirements_2005} 
&The implementation of one requirement causes the increase/decrease of the implementation cost of another requirement.
&If one requirement states that ‘no response time should be longer than 5 seconds, it is most likely to increase the cost of  implementing many other requirements.
%--------------------------------------------------------
\bigstrut\\
\cline{2-5} 
&Increase/Decrease\_value\_of 
& Increase/Decrease\_value\_of~\cite{dahlstedt_requirements_2005} 
& The implementation of one requirement causes the increase/decrease of the value to the customer of another requirement. Note that ‘value’ here mainly reﬂects customer’s satisfaction. 
& Users can listen to MP3 when they are browsing photos in a mobile phone. In this case, ‘users can listen to mp3’ increases
customer’s satisfaction of ‘users can browse photos’. 
\bigstrut\\
\Xhline{4\arrayrulewidth}
%--------------------------------------------------------
\end{tabular}}


==> table_types_zhang_2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\large\resizebox {1\textwidth }{!}{\begin{tabular}{|r|r|r|r|}
\hline
Category &
  Types in Zhang's model &
  Corresponding types  in  other models &
  Example
  \bigstrut\\
\hline
\multicolumn{1}{|c|}{} &
  \multirow{3}[2]{*}{Constrain} &
  \multirow{3}[2]{*}{Constrain ~\cite{k_process_centered_1996}} &
  \multicolumn{1}{l|}{·     r_1: system should respond to users in 3 seconds}
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·      r_2: users search books using book title or ID}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1 constrains r_2}
  \bigstrut[b]\\
\cline{2-4} &
  \multirow{3}[2]{*}{Precede} &
  \multirow{3}[2]{*}{Precondition ~\cite{k_process_centered_1996}, Requires  ~\cite{dahlstedt_requirements_2005}} &
  \multicolumn{1}{l|}{·     r_1: a client initiates a valuation request and the system checks the quality of the request}
  \bigstrut[t]\\
Intrinsic &
   &
   &
  \multicolumn{1}{l|}{·     r_2: users search books using book title or ID}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1 precedes r_2}
  \bigstrut[b]\\
\cline{2-4} &
  \multirow{3}[2]{*}{Be similar  to} &
  \multirow{3}[2]{*}{Similar  ~\cite{k_process_centered_1996}, Similar\_to~\cite{dahlstedt_requirements_2005}} &
  \multicolumn{1}{l|}{·     r_1: a system administrator adds a new book record}
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_2: system administrator modifies an old book record. }
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1 is similar to  r_2 (Book  record  in these  two requirements  is identical).}
  \bigstrut[b]\\
\cline{2-4} &
  \multirow{3}[2]{*}{Conflict} &
  \multirow{3}[2]{*}{Conflicts  ~\cite{k_process_centered_1996}, Conflicts\_with  ~\cite{dahlstedt_requirements_2005}} &
  \multicolumn{1}{l|}{·     r_1: increasing  security}
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_2: improving performance}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1 conflicts with  r_2}
  \bigstrut[b]\\
\cline{2-4} &
  \multirow{3}[2]{*}{Be exception of} &
  \multirow{3}[2]{*}{Only in zhang's model} &
  \multicolumn{1}{l|}{·     r_1: A user inputs a null username and  system  reminds  him to input his correct  username }
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_2: a  user  inputs his  username and  password  and  system checks validity of his information}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1 is an exception of   r_2}
  \bigstrut[b]\\
\cline{2-4} &
  \multirow{3}[2]{*}{Evolve  into} &
  \multirow{3}[2]{*}{Replaces  ~\cite{k_process_centered_1996}, Satisfies  ~\cite{k_process_centered_1996}, Based  on ~\cite{k_process_centered_1996}, Changes} &
  \multicolumn{1}{l|}{·     r_1:  clients  use a desktop  PC  to upload  reports }
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_2:   clients use PDA to upload reports.}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1    evolves into r_2}
  \bigstrut[b]\\
\cline{2-4} &
  \multirow{4}[2]{*}{Refine} &
  \multirow{4}[2]{*}{Refines ~\cite{k_process_centered_1996}, Refines\_to ~\cite{dahlstedt_requirements_2005}} &
  \multicolumn{1}{l|}{·     r_1:  a valuer  submit a valuation report}
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_2:  a valuer  submits a report through web system}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_3:  a valuer  submits a report through PDA}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1 is refined as r_2 and r_3}
  \bigstrut[b]\\
\hline
 &
  \multirow{3}[2]{*}{Increase/Decrease cost of} &
  \multirow{3}[2]{*}{Increase/Decrease\_Cost\-Of~\cite{dahlstedt_requirements_2005}} &
  \multicolumn{1}{l|}{·     r_1:  no response  time  should be longer than  5 seconds}
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1 is most likely to increase  the cost of implementing many  other  requirements. }
  \\
 &
   &
   &
  
  \bigstrut[b]\\
\cline{2-4}Additional &
  \multirow{3}[2]{*}{Increase/Decrease value  of} &
  \multirow{3}[2]{*}{Increase/Decrease\_Value_\Of ~\cite{dahlstedt_requirements_2005}} &
  \multicolumn{1}{l|}{·     r_1:  users  can  listen  to  music  in a mobile  phone}
  \bigstrut[t]\\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_2:   users can  browse  photos in a mobile phone}
  \\
 &
   &
   &
  \multicolumn{1}{l|}{·     r_1    increases customer satisfaction (value) of  r_2}
  \bigstrut[b]\\
\hline
\end{tabular}}%


==> table_types_zhang_3.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
%\Huge
%\huge
%\LARGE
%\Large
%\large
%\normalsize (default)
%\small
%\footnotesize
%\scriptsize
%\tiny
\LARGE
\rowcolors{1}{}{gray}
\resizebox {1.15\textwidth }{!}{\begin{tabular}{|!{\centering}m{4cm}|!{\centering}m{12.8cm}|!{\centering}m{22cm}|!{\centering}m{25cm}|}
		\Xhline{4\arrayrulewidth}
		\textbf{Category} &
		\textbf{Type} &
		\textbf{Description} &
		\textbf{Example}
		%--------------------------------------------------------
		\bigstrut\\
		\Xhline{4\arrayrulewidth}
		intrinsic
		&  Constrain~\cite{zhang_investigating_2014,k_process_centered_1996}  
		& One requirement is a constraint of another requirement. This kind of dependency can represent crosscutting relationships among requirements.
		& \begin{itemize}
			\item $r_1:$ system should respond to users in 3 seconds
			\item $r_2:$ users search books using book title or ID
			\item $r_1$ constrains $r_2$
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\cline{2-4} 
		& Precede~\cite{zhang_investigating_2014}, Precondition~\cite{k_process_centered_1996}, Requires~\cite{dahlstedt2005requirements}
		& If function A precedes function B, A is a precondition of B.
		& \begin{itemize}
			\item $r_1:$ a client initiates a valuation request and the system checks the quality of the request
			\item $r_2:$ users search books using book title or ID
			\item $r_1$ precedes $r_2$
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\cline{2-4} 
		& Be\_similar\_to~\cite{zhang_investigating_2014}, Similar~\cite{k_process_centered_1996}, Similar\_to~\cite{dahlstedt2005requirements}
		&\begin{itemize}
			\item a) If two requirements share similar data information, they are similar to each other. 
			\item b) If two requirements complete similar tasks, they are similar to each other.
		\end{itemize}
		&\begin{itemize}
			\item a) System administrator adds a new book re-cord is similar to system administrator modifies an old book record. Book record in these two requirements is identical. 
			\item b) After a client proposes a property valuation request, one valuer can choose from several options to evaluate the property,such as desktop valuation, curbside valuation or full evaluation Then these options (requirements) are similar to each other.
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\cline{2-4} 
		& Conflicts~\cite{zhang_investigating_2014,k_process_centered_1996}, Conflicts\_with~\cite{dahlstedt2005requirements}
		& Implementation of one requirement negatively impacts another requirement.  
		& \begin{itemize}
			\item Increasing security might negatively impact system performance.
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\cline{2-4} 
		& Be\_exception\_of~\cite{zhang_investigating_2014}
		& One requirement describes an exceptional event of another requirement.
		&\begin{itemize}
			\item $r_1:$ A user inputs a null username and  system  reminds  him to input his correct  username.
			\item $r_2:$ a  user inputs his  username and  password  and  system checks validity of his information.
			\item $r_1$ is an exception of $r_2$. 
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\cline{2-4} 
		& Evolve\_into~\cite{zhang_investigating_2014}, Replaces~\cite{k_process_centered_1996}, Satisfies~\cite{k_process_centered_1996}, Based\_on~\cite{k_process_centered_1996}, Changes\_to~\cite{dahlstedt2005requirements}
		&If requirement B is a new version of requirement A, then A evolves into B. This type of dependency is used
		to trace and compare different versions of requirement documents.
		&\begin{itemize}
			\item $r_1:$ clients  use a desktop  PC  to upload  reports.
			\item $r_2:$ clients use PDA to upload reports.
			\item $r_1$ evolves into $r_2$. 
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\cline{2-4} 
		& Refines~\cite{zhang_investigating_2014,k_process_centered_1996}, Refines\_to~\cite{dahlstedt2005requirements}
		& One requirement is refined by more specific requirements. 
		&\begin{itemize}
			\item $r_1:$ a valuer submit a valuation report.
			\item $r_2:$ a valuer submits a report through web system.
			\item $r_1$ is refined as $r_2$. 
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\hline
		Additional Cost/Value
		& Increase/Decrease\_cost\_of~\cite{zhang_investigating_2014,dahlstedt2005requirements} 
		&The implementation of one requirement causes the increase/decrease of the implementation cost of another requirement.
		&\begin{itemize}
			\item If one requirement states that no response time should be longer than 5 seconds, it is most likely to increase the cost of  implementing many other requirements.
		\end{itemize}
		%--------------------------------------------------------
		\bigstrut\\
		\cline{2-4} 
		& Increase/Decrease\_value\_of~\cite{zhang_investigating_2014,dahlstedt2005requirements} 
		& The implementation of one requirement causes the increase/decrease of the value to the customer of another requirement. Note that value here mainly reflects customers satisfaction. 
		& \begin{itemize}
			\item $r_1:$ users  can  listen  to  music  in a mobile  phone.
			\item $r_2:$ users can  browse  photos in a mobile phone.
			\item $r_1$ increases customer satisfaction (value) of $r_2$. 
		\end{itemize}
		\bigstrut\\
		\Xhline{4\arrayrulewidth}
		%--------------------------------------------------------
	\end{tabular}}

==> table_value.tex <==
\scriptsize\resizebox {0.78\textwidth }{!}{
\begin{tabular}{llllllll}
	\toprule[1.5pt]
	\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{$r_i$}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{$p(r_i)$}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{$v_i$}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{$E(v_i)$}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{$r_i$}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{$p(r_i)$}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{$v_i$}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{$E(v_i)$}} \\ \midrule

	$r_1$ & $00.94$ & $10.00$ & $09.43$ & $r_{15}$ & $00.58$ & 08.00 & 04.64 \\
	$r_2$ & $01.00$ & $20.00$ & $20.00$ & $r_{16}$ & $00.82$ & 10.00 & 08.24 \\
	$r_3$ & $00.37$ & $05.00$ & $01.85$ & $r_{17}$ & $00.12$ & 10.00 & 01.19 \\
	$r_4$ & $00.98$ & $17.00$ & $16.61$ & $r_{18}$ & $00.51$ & 15.00 & 07.59 \\
	$r_5$ & $00.88$ & 06.00 & 05.28 & $r_{19}$ & $00.67$ & 20.00 & 13.41 \\
	$r_6$ & $00.91$ & 20.00 & 18.30 & $r_{20}$ & $00.20$ & 20.00 & 04.09 \\
	$r_7$ & $00.82$ & 15.00 & 12.36 & $r_{21}$ & $00.14$ & 15.00 & 02.05 \\
	$r_8$ & $01.00$ & 09.00 & 09.00 & $r_{22}$ & $00.33$ & 20.00 & 06.59 \\
	$r_9$ & $00.97$ & 20.00 & 19.43 & $r_{23}$ & $00.88$ & 20.00 & 17.61 \\
	$r_{10}$ & $00.76$ & 16.00 & 12.18 & $r_{24}$ & $01.00$ & 01.00 & 01.00 \\
	$r_{11}$ & $00.57$ & 20.00 & 11.36 & $r_{25}$ & $00.24$ & 05.00 & 01.19 \\
	$r_{12}$ & $01.00$ & 12.00 & 12.00 & $r_{26}$ & $00.36$ & 01.00 & 00.36 \\
	$r_{13}$ & $00.76$ & 08.00 & 06.09 & $r_{27}$ & $00.97$ & 05.00 & 04.86 \\
	$r_{14}$ & $00.45$ & 14.00 & 06.28 &  &  &  &  \\[2pt] \midrule
	{\color[HTML]{000000} \textbf{Sum}} & {\color[HTML]{000000} -} & {\color[HTML]{000000} 192.00} & {\color[HTML]{000000} 160.17} & {\color[HTML]{000000} -} & {\color[HTML]{000000} -} & {\color[HTML]{000000} 150.00} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 72.82} \\ \bottomrule[1.5pt]
\end{tabular}

}

==> validation.tex <==
\section{Validation}
\label{ch_dars_validation}




